AIRIVA: A Deep Generative Model of Adaptive Immune Repertoires

Recent advances in immunomics have shown that T-cell receptor (TCR) signatures can accurately predict active or recent infection by leveraging the high specificity of TCR binding to disease antigens. However, the extreme diversity of the adaptive immune repertoire presents challenges in reliably identifying disease-specific TCRs. Population genetics and sequencing depth can also have strong systematic effects on repertoires, which requires careful consideration when developing diagnostic models. We present an Adaptive Immune Repertoire-Invariant Variational Autoencoder (AIRIVA), a generative model that learns a low-dimensional, interpretable, and compositional representation of TCR repertoires to disentangle such systematic effects in repertoires. We apply AIRIVA to two infectious disease case-studies: COVID-19 (natural infection and vaccination) and the Herpes Simplex Virus (HSV-1 and HSV-2), and empirically show that we can disentangle the individual disease signals. We further demonstrate AIRIVA's capability to: learn from unlabelled samples; generate in-silico TCR repertoires by intervening on the latent factors; and identify disease-associated TCRs validated using TCR annotations from external assay data.

==> sections/OLD_discussion.tex <==

The reasoning above holds for the two special cases where there is no confounder, i.e., $\mathbf{c}$ is the empty set, and where $\mathbf{c} = y_2$. However, we find that AIRIVA will fail to generate a valid counterfactual if $y_1$ is the parent of
$y_2$. Given the independence of $z^*_{y_1}$ from  all other dimensions of $\zv$ in the graphical model, AIRIVA does not model the effect of $y_1$ on $y_2$. Furthermore, we assume that $\xv$ is always only an effect, never a cause.

==> sections/cohort.tex <==
% \emph{This section is optional, and more theoretical work may not need this section.  However, if you are using health data, then you need to describe it carefully so that the clinicians can validate the
%   soundness of your choices.} 

% Describe the cohort.  Give us the details of any inclusion/exclusion criteria, what data were extracted, how features were processed,
% etc.  Recommended headings include:

% \subsection{Cohort Selection} 
% This includes choice of criteria and basic numbers, as well as any relevant information about the study design (such how cases and controls were identified, if appropriate), 

% \subsection{Data Extraction} 
% This includes what raw information you extracted or collected, including any assumptions and imputation that may have been used, and 

% \subsection{Feature Choices} 
% This includes how you might have converted the raw data into features that were
% used in your algorithm. 

% Cohort descriptions are just as important as methods details and code to replicate a study.  For more clinical application papers, each of the sections above might be several paragraphs because we really want to understand the setting.

% For the submission, please do \emph{not} include the name of the institutions for any private data sources.  However, in the camera-ready, you may include identifying information about the
% institution as well as should include any relevant IRB approval statements.
\section{Datasets}\label{sec:cohort}

%\MFP{@Rebecca and @Steven: Where do the repertoire labels come from (clinical tests?), why are there missings in the HSV dataset? What is the goal/challenge in each of these datasets, and why do current approaches such as ESLG struggle? Optionally, discuss past work of Rebecca on COVID that did rely on MIRA hits to do careful TCR selection, whereas we build a robust model for disease diagnostic without requiring any expensive annotations.}

\subsection{COVID-19}
The viral envelope of SARS-CoV-2 is made up of three proteins: the membrane protein, the envelope protein, and the spike protein. The spike protein is believed to be responsible for binding to host cells and initiating viral infection, and has therefore been the target of vaccine development. During natural infection, we expect to see expansion of TCRs associated with any one of these proteins, while in the case of vaccination\footnote{We consider viral vector vaccines AZD1222 (Oxford-AstraZeneca) and Ad26.COV2.S (Johnson \& Johnson), as well as mRNA vaccines BNT162b2 (Pfizer) and mRNA-1273 (Moderna).} we should only observe expansion of TCRs binding the spike protein. We would like to build a model that can disentangle natural infection from vaccination. Because TCRs clonally expanded during natural infection are a superset of the spike-only TCRs expanded following vaccination, this is a challenging task.

To train our models we used $1,954$ samples from donors with natural SARS-CoV-2 infection, $477$ healthy donors post SARS-CoV-2 vaccination, and $5,198$ healthy controls sampled prior to March 2020. The classifiers are tested on a holdout set of $525$ samples from naturally infected donors, $400$ vaccinated donors, $100$ donors who were naturally infected and later vaccinated, and $4606$ healthy controls.

Prior work with these data have utilized a large database of TCR-antigen pairs generated by multiplexed antigen stimulation assays (MIRA) \citep{klinger2015multiplex}. By intersecting public COVID-19-associated TCRs with this database, it is possible to associate a subset of the TCRs to an antigen (spike or non-spike) with high confidence \citep{Li2022}. However, generating such a database of TCR-antigen pairs is a time-intensive and expensive endeavor. Therefore, a method that can disentangle antigen-specific T-cells without the need for costly experiments is highly desirable. 

We posit $\yv = \{\yvs_\text{ns}, \yvs_\text{s}, \yvs_\text{depth}\}$, where $\yvs_\text{ns}$ and $\yvs_\text{s}$ refer to exposure to the non-spike and spike proteins respectively, and $\yvs_\text{depth}$ refers to sequencing depth---a standardized measure of log total template count---as there is a strong depth imbalance between the vaccinated subpopulation and others (see Appendix for details). For $\yvs_\text{ns}$ naturally infected samples are positives and vaccinated and healthy controls are negatives. For $\yvs_\text{s}$ both naturally infected and vaccinated samples are positives and healthy controls are negatives. 


\paragraph{External Spike and Non-Spike Annotations}\label{sec:mira}
\TM{merge with 3rd para} In addition to repertoire-level labels, in the case of COVID-19 we have access to in-vitro labels for spike and nonspike TCR associations from external MIRA (\textbf{M}ultiplexed \textbf{I}dentification of T cell \textbf{R}eceptor \textbf{A}ntigen specificity) assay data~\citep{klinger2015multiplex}.
This data comprises over 400k experimentally-derived TCR-antigen binding pairs (\emph{hits}) for the spike protein, and 1.2M hits for non-spike proteins~\citep{nolan2020large}.
% Of these, 291 spike and 462 nonspike associated TCRs appear in our set of 1596 TCRs from FET used as input to AIRIVA.
%Of these, 75 spike and 105 nonspike associated TCRs appear in our set of 612 TCRs from FET used as input to AIRIVA.
% We have 422,933 MIRA hits for spike, and 1,238,238 for nonspike, of which 19,006 MIRA hits for spike and 50,050 for nonspike appear in at least 10\% of the covid-positive cases in the repertoire data. 
We use these spike and non-spike protein specific TCRs from MIRA to assess the quality of learned TCR-label associations from AIRIVA.
%, and compare against group mean differences between cases and controls.



% \begin{figure}[h!]
% 	\centering
%  %\includegraphics[width=\linewidth]{figures/final/mira_covid.png}
%  %\includegraphics[width=\linewidth]{figures/final/ates.png}
% 		\includegraphics[width=0.3\textwidth]{figures/final/mira_covid2b.png}
% 		\caption{Underlying data structure for COVID-19.}
% 		\label{fig:covid_data_structure}
% \end{figure}
%
 %We thus posit $\yv = \{\yvs_\text{ns}, \yvs_\text{s}, \yvs_\text{depth}\}$, where $\yvs_{ns}$ and $\yvs_s$ refer to exposure to the nonspike and spike proteins respectively, and $\yvs_\text{depth}$ refers to sequencing depth as described above.

\subsection{Herpes Simplex Virus}
%
%\paragraph{Dataset description}
HSV-1 and HSV-2 are two members of the Herpes Simplex Virus (HSV) family. The two viruses share approximately 80\% of their genome~\citep{greninger2018ultrasensitive}, and will therefore have partially overlapping antigen sets and corresponding TCRs, making it challenging to build a model which accurately disentangles their labels.
Infections for both are frequent in the population, with $\approx$ 67\% prevalence for HSV-1 and $\approx$ 13\% prevalence for HSV-2~\citep{james2020herpes}. Infection status for either virus is independent of the other and infections frequently co-occur. Our dataset consists of samples labeled for both HSV-1 and HSV-2 using multiplexed IgG serology. The dataset comprises a total of 1125 repertoires in the training set, and 289 in the test set. We are unable to confidently assign a label for HSV-1 and/or HSV-2 in roughly 20\% of our samples. We include these unlabeled samples for AIRIVA in a semi-supervised context. Here we build an AIRIVA model to disentangle the two labels. We posit the set of labels $\yv = \{\yvs_\text{hsv1}, \yvs_\text{hsv2}\}$.\footnote{There is no depth imbalance in this dataset, so adding a depth label to AIRIVA is not needed.}
% \MFP{Add tables with numbers per subgroup and a sentence re missings, probably in Appendix, what s the percentage of unlabelled repertoired, etc}.
%
%In addition to $\yvs_\text{hsv1}$ and $\yvs_\text{hsv2}$, we provide depth as an additional label $\yvs_\text{depth}$---a standardized measure of log total template count---as depth is often a source of bias in repertoire disease classification.
%
  %Note that we do not posit a label for depth in contrast to the COVID-19 application, as the number of input TCRs considered for HSV is small, making it challenging to predict repertoire depth from just a few.
%
%Full details of the datasets are available in the Appendix.

%\paragraph{HSV}
%Our dataset consists of 1003 repertoires with 451 HSV-1 only positives, 74 HSV-2 only positives, 223 samples that are positive for both and 255 that are positive for neither. We split our data 80:20 for model training and validation. In addition we have a holdout set of 241 samples only used for evaluation. We filter TCRs by a one-sided FET as described above for each binary label down to a p-value threshold of 3e-4. This gives us a total set of 325 sequences. Because of the overlapping binary labels we expect these sequences to be a mix of HSV-1 specific, HSV-2 specific and shared TCRs. 

==> sections/fig_assumed_causal_graph.tex <==
\begin{figure}[]
%\begin{minipage}[b]{0.5\linewidth}
    \centering
    \caption{\textbf{Assumed causal graph}: AIRIVA assumes that data comes from a disentangled causal process, a specific family of causal graphs where the true factors of variation $Y_1, \ldots, Y_K$ cannot cause each other. Here, the observed TCR counts repertoire $\xv$ results from the combination of factors $\yv$, i.e., exposures to certain antigens, age, genetic factors, etc. which may be correlated by unobserved confounders $\cv$ but do not cause one another. %We further assume that no factor causes another.
    }\label{fig:causal}
    \begin{tikzpicture}[x=1.8cm,y=0.5cm]
        \node[latent]                              (c)      {$\cv$} ; %
        \node[latent, below=of c, xshift=1cm]      (y2)     {$Y^2$} ; %
        \node[latent, left=of y2]                  (y1)     {$Y^1$} ; %
        \node[latent, right=of y2]                 (yk)     {$Y^K$} ; %
        \node[latent, below=of y2]                 (x)      {$\xv$};
        \path (y2) -- node[auto=false]{\ldots}     (yk);
        \edge {c} {y1,y2} ; %
        \edge {y1,y2,yk} {x} ; %
    \end{tikzpicture}
    %\includegraphics[width=1.0\linewidth]{figures/causal_graph.png}
	
 % \includegraphics[width=\linewidth]{diagrams/diag_simplified.png}
	% \includegraphics[width=\linewidth]{diagrams/moonshot.png}
    % \includegraphics[width=0.7\linewidth]{figures/final/goal_work.png}
    % \includegraphics[width=0.75\linewidth]{figures/final/intro_pgm2.png}
    	% \caption{\textbf{Goal of this work}: we propose a deep generative model to decompose the adaptive immune response signal and estimate causal effects in the context of TCR count data. The inferred latent factors are human-interpretable and can be manipulated to simulate in-silico repertoires and counterfactuals, enabling downstream applications such as identification of disease-specific TCRs.
    % identify disease-specific TCRs by disentangling the TCR immune response in compositional latent factors which can be intervened on to estimate counterfactuals and causal effects. We assume the above causal graph for our data: the observed TCR counts $x$ result from a combination of elementary factors $g_1, g_2, \cdots, g_k$, which may be correlated by unobserved confounders $c$, and such that no factor is a parent of another.
%\end{minipage}
%\begin{minipage}[b]{0.5\linewidth}
%\end{minipage}
\end{figure}

==> sections/fig_data_flow_cf.tex <==
% \begin{figure}[t!]
% \centering
%     \caption{Data flow to generate counterfactuals with AIRIVA in an example with two labels. Counterfactuals are generated for a data point in which $y_1$ is set to $y_1^*$. \MFP{(TODO: font bigger, adapt notation to be consistent with text).}
%     } \label{fig:ctf}
%      \includegraphics[width=0.4\linewidth]{diagrams/counterfactuals.png}
% \end{figure}
% \begin{figure}[t!]
%     \centering
% 	\includegraphics[width=1.0\linewidth]{diagrams/counterfactuals.png}
%     \caption{Data flow to generate counterfactuals with AIRIVA in an example with two labels. Counterfactuals are generated for a data point in which $y_1$ is set to $y_1^*$.
%     %{\color{red}(TODO: adapt notation in diagram to be consistent with text).}
%     }
%     \label{fig:ctf}
% \end{figure}

==> sections/introduction.tex <==
T cells are the adaptive immune system’s first line of defense against immune-mediated diseases, i.e. infectious diseases, auto-immune diseases and cancer~\citep{collier2021not}. %Figure~\ref{fig:intro-antigen1} illustrates the in-vivo generative process of the immune repertoire of an individual.
When an individual is exposed to a disease, only those T cells with T-cell receptor sequences (TCRs) binding the disease antigens undergo clonal expansion. After clearing of the disease, TCRs persist in immunological memory. At any given time, a snapshot of TCRs in an individual comprises a mix of current and past disease states, as well as naive TCRs that have yet to encounter their cognate antigen. A TCR repertoire, equivalent to a bag of words in a document, is a subsample of the complete set of TCRs in an individual.
\TM{I don't think this is the reference we want.  Something from adaptive instead?  Or AIRR?}
TCR repertoires can be efficiently assayed based on targeted high-throughput sequencing given a standard blood sample~\citep{pavlovic2022using}, opening the door to a new form of precision diagnostic based on adaptive immune repertoires.

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.7\linewidth]{figures/intro/fig1_diseases.png}
    
%      \caption{
%      Illustration of the in-vivo generative process of immune repertoires. When a T-cell binds to a specific molecular structure or \textit{antigen}, it undergoes clonal expansion (A), which is indirectly captured in a blood sample (B) and quantified using high-throughput immuno-sequencing resulting in a TCR repertoire (C).
%     }
%     \label{fig:intro-antigen1}
%     \vspace{-0.5cm}
% \end{wrapfigure}


% set of TCR sequences with high counts (histogram). A TCR repertoire, equivalent to a bag of words in a document, is a subsample of the complete set of TCRs in an individual.
%TCR repertoires are high-dimensional molecular markers reflecting past and present immune responses of a patient, which can be efficiently assayed based on targeted high-throughput sequencing given a standard blood sample~\cite{pavlovic2022using}.
%
%Next-generation sequencing technologies have made it possible to directly probe the functional nature of T-cells by sequencing an individual’s TCR repertoire from a blood sample.
%
Recent works have shown promise in building models based on TCR repertoires to detect current or past infection for several diseases, including Cytomegalovirus~\citep{emerson_immunosequencing_2017}, Lyme disease~\citep{greissl2021immunosequencing}, and COVID-19~\citep{snyder2020magnitude}.
%
As we consider building a model that captures our knowledge of the adaptive immune response, it is crucial to account for the challenging complexity of immune repertoires and the data generated from collections of repertoires.

%A TCR repertoire, equivalent to a bag of words in a document, is a subsample of the complete set of TCRs in an individual. It is highly heterogenous, depending on exposure history but also genetic factors, sequencing depth and experimental effects. 

% T-cells play an important role in identifying and fighting viral infections, and are thought to be critical mediators of response in autoimmune disease and cancer \citep{collier2021not}
%, making them a promising route to improved diagnostics in these settings.
% The adaptive immune repertoire is highly diverse, with $O(10^7)$ unique TCRs in any given individual, drawn from a much larger pool of possible sequences.
% When exposed to certain disease antigens, TCRs with high affinity to these antigens stimulate the T cell to undergo clonal expansion; for a disease of interest only a small fraction of these TCRs are specific to the disease.
% Recent advances in high-throughput immune repertoire sequencing have laid the foundation for a new form of precision diagnostic based on T-cell receptor (TCR) signatures.
%
%The adaptive immune system is a powerful framework to fight disease, with diverse receptors that can recognize a large variety of diseases and self-antigens.
%
%Within the adaptive immune system,


% %Recent works in immunomics have introduced a new form of precision diagnostic based on T-cell receptor (TCR) signatures, showing promise in detecting new or past infection based on TCR signatures for several diseases, including Cytomegalovirus~\cite{emerson_immunosequencing_2017}, Lyme~\cite{snyder2020magnitude}, and COVID-19~\cite{greissl2021immunosequencing}.
% %
% %When exposed to disease antigens, only those T-cells with T cell receptors (TCRs) with high affinity to those antigens undergo clonal expansion.
% %
% %The high specificity of TCRs to disease antigens opens the door to a new form of precision diagnostic based on adaptive immune repertoires.
% %
% Immune repertoires, comprising all T and B cells in the body, reflect past and present immune responses, opening the door to a new form of precision diagnostic.
% %and can be assayed via high-throughput sequencing from a blood sample.
% %
% %We call TCR \textit{repertoire} the collection of TCRs present for a given individual.
% %TCR repertoires are "high-dimensional molecular markers reflecting past and present immune responses of a patient and can be efficiently assayed based on targeted high-throughput sequencing from a standard blood sample".
% %
% Recent works have shown promise in building models based on T-cell receptor (TCR) repertoires to detect new or past infection for several diseases, including Cytomegalovirus~\cite{emerson_immunosequencing_2017}, Lyme disease~\cite{greissl2021immunosequencing}, and COVID-19~\cite{snyder2020magnitude}.
% %
% As we consider building a model that captures our knowledge of the adaptive immune response, it is crucial to account for the challenging complexity of immune repertoires and the data generated from collections of repertoires.

 
%Figure~\ref{fig:intro-antigen1} illustrates the in-vivo generative process of the immune repertoire of an individual. When a T-cell binds to a specific molecular structure or \textit{antigen}, it undergoes clonal expansion (A), which is indirectly captured in a blood sample (B) and quantified using high-throughput immuno-sequencing, resulting in (C), a set of TCR sequences with high counts (histogram). TCR counts provide a look to past and present immune responses of an individual given a blood sample~\cite{pavlovic2022using}.

\begin{figure*}[]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/intro/fig1_intro.png}
     \caption{Data flow and representation in AIRIVA. (A) inputs are a fixed set of TCR counts per repertoire; targets
are presence of different diseases (binary), and sequencing depth (continuous). (B) AIRIVA maps TCR repertoires to independent latent factors.
%, i.e., single scalar factors per genetic and disease targets.
(C) In-silico repertoires can
be generated by switching on and off targets or toggling sequencing depth. %\MFP{TODO: eps format, change to "covariate factor" instead of just diseases.}
    }
    \label{fig:intro-antigen2}
\end{figure*}

TCR repertoires are highly heterogeneous and diverse, with $O(10^7)$ unique TCRs in any given individual~\citep{emerson_immunosequencing_2017}, which makes it challenging to disentangle disease-specific factors from noise and undesired biases~\citep{teschendorff2019avoiding}.
Several factors beyond the disease contribute to clonal expansion of TCRs. Such factors include genetic markers, past infections, correlations in antigen exposure or endemic diseases in a particular region, as well as undesired effects arising from the assay chemistry.

One key genetic factor in TCR-antigen binding and the resulting repertoire is the human leukocyte antigen (HLA). HLAs are cell surface receptors that bind disease antigens and present these to T-cell receptors. HLAs are heritable, highly polymorphic and because of antigen presentation, directly influence an individual’s TCR repertoire. In some auto-immune diseases such as celiac disease, HLAs can act as confounders because they directly influence disease risk. 
%
Sequencing depth, i.e. the number of TCRs in a repertoire, can vary considerably between samples. Such variation are caused by multiple reasons, including experimental protocol or biological factors related to age or specific illnesses. Since disease signal naturally increases with depth as more TCRs associated with disease emerge in the sample, accounting for sequencing depth is essential for not only realistic in-silico sample generation, but for robust disease classifiers that perform well across all depths.

%, yielding undesired confounding bias.
%%Identifying the disease-specific TCRs in the presence of these confounders and such high-dimensional data is like finding a bunch of needles in a haystack.
%Accounting for these various genetic/experimental/batch effects in the underlying data-generating process is crucial to avoiding spurious correlations and developing robust diagnostics.
%\TM{dont shy away deeper explanations of challenges as bulk on intro}

%An effective simulator of TCR repertoires (the set of TCRs in an individual) addresses many of these challenges. However, as with all simulators, we are interested in knobs that control, ideally, independent factors in the data generating process. In our immunomics application, these knobs include not only the disease indicator and the genetic risk factor(s), but also the sequencing depth.

With the goal of learning a \emph{data-driven} simulator with knobs for controlling independent factors of variation in immunomics, we build on generative models that explicitly focus on learning disentangled latent representations. The underlying assumption is that sets of antigens drive TCR expansion independently from each other.
%
%Generative models give us three main advantages with respect to current approaches that only aim to classify the disease without further considerations. First, using a generative model allows to generate in-silico repertoires that can be used to correct for distribution imbalance guard against domain shifts. Second, generative models allow us to learn from unlabelled samples, which reduces the need for collection of expensive labels. Third, learning a disentangled latent representation enables scientific discovery of biological insights, including the identification of label-specific TCR associations.
%
Figure~\ref{fig:intro-antigen2} summarizes the key idea and intuition behind this work. We present the \textit{Adaptive Immune Repertoire-Invariant Autoencoder} (AIRIVA), a probabilistic framework that takes as input (A) a collection of TCR count immune repertoires along with relevant repertoire labels, (B) to learn a disentangled latent representation of TCR repertoires. Once AIRIVA has been trained, we can (C)~generate in-silico repertoires by intervening on the latent factors, providing new avenues for understanding the key aspects that underpin the adaptive immune
response.

AIRIVA provides several advantages over traditional classification-based approaches. First, it allows for the generation of in-silico repertoires, which can correct for distribution imbalance and guard against domain shifts. Second, it can learn from unlabelled samples, allowing us to leverage more data without the need for expensive disease annotation across all repertoires. Third, the learnt representation enables the discovery of label-specific TCR associations, and elicit new biological insights.


\subsection*{Generalizable Insights about Machine Learning in the Context of Healthcare}
%This section is \emph{required}, must keep the above title, and should be the final part of your introduction.  In about one paragraph, or 2-4 bullet points, explain what we should \emph{learn} from reading this paper that might be relevant to other machine learning in health endeavors. For example, a work that simply applies a bunch of existing algorithms to a new domain may be useful clinically but doesn't increase our understanding of the machine learning and healthcare; if that study also investigates \emph{why} different approaches have different performance, that might get us excited!  A more theoretical machine learning work may be in how it enables a new kind of clinical study. \emph{Reviewers and readers will look to evaluate (a) the significance of your claimed insights and (b) evidence you provide later in the work of you achieving that contribution}
\TM{highlighting importance of this section which should be prioritized}
This work explores the use of invariant deep learning in immunomics, a field that has the potential to revolutionize the way precision medicine is done. We develop AIRIVA, a deep generative model for TCR repertoires, that corresponds to the adaptation of recent work~\citep{ilse2020diva, joy2020capturing} to immunomics.
%to model immunomics data that comprise TCR repertoires for multiple patients and several labels (\emph{e. g.}, disease, risk and depth) and cohorts that may have been collected for several reasons.
%The model is general, as described in Section~\ref{sec:methods}, and it is an adaptation of the work by~\citep{ilse2021selecting} to immunomics.
%
We propose a procedure to generate in-silico repertoires  with AIRIVA by manipulating specific latent factors of interest, and make a link to the classical way of generating counterfactuals in causal inference.
%\item A procedure to generate counterfactual repertoire data with AIRIVA, which allows to intervene and generate \emph{in silico} repertoires by acting on different factors of interest. We review the connections of this way of sampling synthetic data with the classical way of generating counterfactuals in causal inference.
Finally, we empirically demonstrate AIRIVA’s capacity to disentangle disease signal in the context
of two infectious diseases, COVID-19 and Herpes Simplex Virus, improving model robustness across subgroups of interest. Overall, AIRIVA provides a powerful tool for analysing TCR repertoires, for both diagnosis and scientific discovery.
%, validated using external experimental data.
%\item New results and insights in a real dataset of patients with Multiple Sclerosis. Using a baseline logistic regression model to classify patients, we show that training the classifier on augmented synthetic data improves generalization due to the balancing (bias reduction) effect of the counterfactuals have in the training process. Counterfactual data are also interpretable, which increase the transparency in our analysis and opens the door to new biological insights.

%We apply AIRIVA to two infectious disease contexts: COVID-19 (natural infection and vaccination) and Herpes Simplex Virus (HSV-1 and HSV-2), and empirically show that we can disentangle disease signal from these labels for prediction, improving model robustness across subgroups of interest. We demonstrate AIRIVA's ability to: generate realistic in-silico TCR repertoires conditioned on specified labels by intervening on the learnt latent factors, learn from unlabelled repertoires, and identify disease-associated TCRs, validated using TCR annotations from external assay data. Overall, AIRIVA provides a powerful tool for analysing TCR repertoires, for both diagnosis and scientific discovery.

%The discovery of relevant biomarkers in the presence of undesired biases is central to learning from high-dimensional, heterogenous \emph{-omics} data.


==> sections/litreview_bio.tex <==
\subsection{TCR-based Methods for Disease Diagnosis.}

The ability of the adaptive immune system to recognize and fight infection relies on the T-cell receptors (TCRs) expressed on the surface of T-cells. Typically, TCR repertoires in healthy adults have of the order of $10^7$ unique TCRs, drawn from a much larger pool of possible sequences~\citep{emerson2017immunosequencing}. These TCRs are specific to a given disease antigen; when exposed to an antigen of interest, these T cells are activated and undergo clonal expansion, some remaining for years as memory cells. These clonally expanded TCRs can be used as the basis of disease diagnosis, such as in the case of cytomegalovirus (CMV,~\cite{emerson2017immunosequencing}), Lyme disease \citep{greissl2021immunosequencing}, or COVID \citep{gittelman2021diagnosis}. \dots

% TODO: Add further references @Rebecca?
%\begin{itemize}
%	\item \cite{emerson2017immunosequencing} Detection of CMV infection using TCRs.
%	\item \cite{snyder2020magnitude} Detection of SarsCov2 using TCRs.  Related \cite{elyanow2021t}
%	\item \cite{greissl2021immunosequencing} Detection of Lyme using TCRs.
%\end{itemize}
%\paragraph{Undertanding COVID response using TCR Repertoires}
%\cite{elyanow2022t, minervina2021longitudinal,luo2021dynamics}




==> sections/litreview_ml.tex <==
\paragraph{Machine Learning Models for Immunomics} 
Recent advances in sequencing technologies have increased the availability of TCR sequencing data and enabled the training of deep learning models \cite{annurev-chembioeng}. These include for example DeepTCR \citep{sidhom2021deeptcr}, which uses deep VAEs of TCR sequences to learn features useful for antigen binding prediction and repertoire classification using a multiple instance learning framework, and DeepRC \citep{widrich2020modern}, which incorporates Hopfield networks into BERT transformers to classify repertoires in the context of existing metadata. Despite these efforts, L1 penalized logistic regression has been proven to achieve the highest prediction performance on TCR repertoire data \citep{kanduri2022profiling, emerson2017immunosequencing}.

AIRIVA differs from existing deep learning frameworks trained on TCR repertoire data in several key ways: while the primary goal of models such as DeepTCR and DeepRC is prediction of TCR-antigen binding, based on TCR sequence information, here we focus instead on learning disentangled factors of variation that enable in-silico repertoire generation, taking TCR counts as input.


% Advances in sequencing technologies have lead to an increase of the availability of TCR sequencing data, making it possible to train deep learning models~\cite{annurev-chembioeng}.
% %
% Although AIRIVA is trained on TCR repertoire data using a deep learning framework, the goal of our model---disentangle disease-associated TCRs and generate repertoires---differs from most other deep learning models in the field. The most similar approaches are DeepTCR~\citep{sidhom2021deeptcr} and DeepRC~\citep{widrich2020modern}. DeepTCR uses deep VAEs of TCR sequences to learn features useful for antigen binding prediction and repertoire classification using a multiple instance learning framework. DeepRC incorporates Hopfield networks into BERT transformers to classify repertoires in the context of existing metadata. Despite these efforts, L1 penalised logistic regression has been proven to achieve the highest prediction performance on TCR sequencing data~\citep{kanduri2022profiling, emerson2017immunosequencing}.
% While the primary goal of those works is prediction, we focus on learning disentangled factors of variation that enable in-silico repertoire generation via label conditioning or counterfactuals. %To the best of our knowledge, AIRIVA is the only model to disentangle disease-specific TCRs based on repertoire-level labels and to generate counterfactual data.

%\vspace{-0.3cm}
%\paragraph{Learning independent factors of variation with deep generative models}
\paragraph{Generative Models for Disentanglement}
Recent state-of-the-art generative models leverage amortized variational inference \citep{kingma2013auto, rezende2014stochastic} to identify independent factors of variation in data \citep{locatello2019challenging, kim2018disentangling}. \citet{joy2020capturing} and \citet{ilse2020diva} have developed generative models that learn label-specific independent factors of variation from labelled data. AIRIVA adapts the recently proposed DIVA framework \citep{ilse2020diva} to the adaptive immune repertoire dataset and demonstrates a novel use of DIVA, for in-silico conditional and counterfactual repertoire generation, and inference of TCR-label associations based on conditional ATEs, moving beyond domain-invariant prediction. Disentanglement in a generative model has been shown to be impossible without access to labels \citep{kim2018disentangling,locatello_challenging_2019}; in this work, we use repertoire-level labels to guide the inference of human-interpretable latent factors and generate in-silico repertoires with specific characteristics.

% AIRIVA adapts the recently proposed  DIVA framework \citep{ilse2020diva} to the adaptive immune repertoire dataset, and shows a novel use of DIVA for valid counterfactual generation and estimation of multi-output average treatment effects. Note that disentanglement in a generative model has been shown to be impossible without access to labels \citep{kim2018disentangling,locatello_challenging_2019}. In this work, we use repertoire-level labels to guide the inference of human-interpretable latent factors, and to generate in-silico repertoires with specific characteristics.
%Note that disentanglement in a generative model is impossible without access to labels \citep{kim2018disentangling,locatello_challenging_2019}.
%

% \vspace{-0.3cm}
% \paragraph{Counterfactual Generation}
% Counterfactual inference has been explored extensively for heterogeneous treatment effect estimations of binary or continuous potential outcomes given covariates and intervening treatment, see \citep{johansson2016learning, shalit2017estimating, shi2019adapting, vlontzos2021estimating, assaad2021counterfactual, yoon2018ganite}.
% %
% Most previous approaches focus on potential outcome predictions for causal effect estimations. In contrast, our work leverages amortized inference using a deep generative model with a factorized latent representation which attempt to learn independent factors of variation of the data.
% %
% Especially related to our work are methods that factorise the latent space into independent risk, confounding, and instrumental factors \citep{hassanpour2019learning, vowels2021targeted, kuang2017treatment, zhang2020treatment}. In contrast to these works, we assume a much simpler scenario where the true data generating process is a causal disentangled process as described in~\cite{suter2019robustly}. %independent as in Figure~\ref{fig:intro}.
% %we leverage both counterfactual and factual data generation for augmenting the training data set of the outcome prediction task: as described, we generate counterfactual data by intervening on the learned disentangled representation of the TCRs. Thus, our generative model can be used for robust disease prediction as the augmented data exhibits weaker confounding biases \citep{suter2019robustly, ilse2021selecting}.


==> sections/methodology-old.tex <==

%=========================================================================================



%\section{METHODS}\label{sec:methods}

%Key argument for the story. One model for two tales: robust classification
%(disease diagnostic) and counterfactuals generation (interpretability) in the
%same place. These also reinforce each other: by generating counterfactuals (fake
%data), in these are correct by retraining the model using factual and
%counterfactuals should be correct selection bias and make the model predict
%better in other cohorts. How to do it: Bayesian Deep learning – CCVAE-DIVA
%inspired model:

CCVAE \citep{joy2020rethinking}


%\subsection{The Enhanced Sequence Invariant Variational Autoencoder (ESIVA)}\label{sec:ESIVA}

%\begin{itemize}
 %   \item high dimensional data setting ($d>>n$), not enough data for reasonable
%          hyperparameter tuning
%\end{itemize}


%\subsection{Training of DIVA}
\paragraph{Generative Model}
For $\dss$ denoting the disease variable, and $\tcr$, the generative model of DIVA currently
looks like this
$$p(z_{\dss}|\dss)\prod_{i=1}^{20} p(z_{\hla_i}|\hla_i)p(z_{\depth}|\depth)p(z_{residual})p(\tcr|z_{\dss},
    z_{\hla}, z_{\depth}, z_{residual})$$
where
\begin{align*}
    z_{\dss}|\dss \sim N(\mu_{\dss}, \sigma_{\dss}), \text{ }
    z_{\hla_i}|\hla_i \sim N(\mu_{\hla_i}, \sigma_{\hla_i}), \text{ for }i\in\{1,..., 20\}
    z_{\depth}|\dss \sim N(\mu_{\depth}, \sigma_{\depth})
\end{align*}
top 20 HLAs chosen as those HLAs with the highest difference in frequency

\paragraph{Inference Model}
For $\dss$ denoting the disease variable, and $\tcr$ the TCRs, the generative model of DIVA currently
looks like this
$$
    q(z_{\dss}|\tcr)q(z_{\depth}|\tcr) p(\depth|z_{\depth}) \prod_{i=1}^{20} q(z_{\hla_i}|\tcr) p(\hla_i|z_{\hla_i})
$$



\subsection{Counterfactuals generation}\label{sec:counterfactuals}

\begin{itemize}
    \item Detail here the algorithm used to generated counterfactuals.
    \item This can be a good place to show the counterfactual paths, and their consistency.
\end{itemize}

\subsection{Data augmentation and bias reduction}\label{sec:data_augmentation}

\begin{itemize}
    \item Provide some statistical arguments of why counterfactual augmentation works. Arguments about bias reduction, etc.
    \item Explain why the invariances imposed in ESIVA make the simulated data to be real cunterfactuals.
\end{itemize}

\subsection{Domain invariant variational autoencoder}

GANs cannot model count data. Regression-like models cannot capture the
dependency in the high-dimensional covariate space.

\subsection{Counterfactual Generation}
Pearl’s ladder of causation \citep{pearl2019seven} describes three types of
distributions that can be used to generate a data point $X$ given covariates
$y$: association $P(X|Y = y)$, intervention $P(X| \judo(Y = y))$ and
counterfactual $P(X_{Y=y}|Y = y', X = x').$.

Conditional generative models such as conditional GANs or conditional VAEs are
typically limited to modeling associational distributions. \unsure{In a case
    where $y$ causes $X$, $X$ has no (indirect) effect on $y$, and $X$ and $y$ are
    not confounded, conditional models can also model the interventional case.} In
this work, we want to focus on the third level: counterfactual generation.

\cite{pearl2019seven}
\begin{enumerate}
    \item \textbf{Abduction}: Infer latent $z$ given the input $(x, a)$ using
          the encoder.
    \item \textbf{Action}: Let $a_k \subseteq a$ be the set of $k$ attributes
          that one wants to intervene on. Set attribute $a_i\rightarrow a'_i
              \forall a_i\in a_k$, given $a'_k=\{a'_i\}_{i=1}^k$
    \item \textbf{Prediction}: Modify all the descendants of $a_k$ according to
          the SCM equations learned by Attribute-SCM. This outputs $a_c$, the
          intervened attributes. Use $z$ from the encoder and $a_c$ from the
          Attribute-SCM and input it to the generator to obtain the
          counterfactual $x_c$
\end{enumerate}

In contrast to \cite{pawlowski2020deep} we do not sample from the quantiles
since we observed unstable behaviour. \unsure{This can be explained by the
    difficulty of training calibrated decoders \cite{rybkin2021simple}}.

\subsection{Shared DIVA extension}
inspired by doubly robust methods: we model exposure model and treatment model


%Key argument for the story. One model for two tales: robust classification (disease diagnostic) and counterfactuals generation (interpretability) in the same place. These also reinforce each other: by generating counterfactuals (fake data), in these are correct by retraining the model using factual and counterfactuals should be correct selection bias and make the model predict better in other cohorts.
%How to do it: Bayesian Deep learning – CCVAE-DIVA inspired model:

%Importance of Data augmentation
%\begin{itemize}
%    \item high dimensional data setting ($d>>n$), not enough data for reasonable hyperparameter tuning
%\end{itemize}

%Why? Apart from predictive performance, why is this a more foundational way to solve the problem:
%\begin{itemize}
%    \item Allows for data exploration and visualization via the latent space.
%    \item (Partially) generative model -> Counterfactual generation -> interpretability + synthetic data.
%    \item Natural way to expand repertoires of indicators to counts, sequences, etc. Perhaps we don’t want to talk to %much about this if we are not going to show anything with sequences.
%    \item Natural extension to multiple labels.
%    \item Invariant representation robust against the inclusion of non-causal TCRs.
%    \item can be extended to differentially private setting if useful
%\end{itemize}
%
%Model novelties, developed for the current application:
%\begin{itemize}
%    \item Work of different ways of constructing the latent in terms of the causal assumptions (is this really needed?)
%    \item Counterfactuals: model uncertainty and develop a validation strategy: (i) use synthetic data generated using %another generative model (ii) generate synthetic data, retrain the model and check generalization in other cohorts), (iii) %search for optimal matching methods in the datasets (iv) use the MIRA data.
%    \item Uncertainty quantification on the counterfactuals.
%    \item Other? Priors on the counts, etc? hint on how to do this for sequences?
%    \item Theoretical connections with other forms of invariances? Connections between the imposed disentanglement in %the latent space and the causal assumptions.
%\end{itemize}
%This is needed to justify that the synthetic data generated with the model are really counterfactuals.
%
%Toy Figures
%\begin{itemize}
%    \item trajectory of counterfactuals that Ted proposed
%\end{itemize}



==> sections/methods_exp_old.tex <==
In this section, we describe experiments to empirically demonstrate the capacity of AIRIVA to (i) generate in-silico TCR repertoires with manipulable characteristics, (ii) identify disease-specific TCRs in the presence of confounding, and (iii) correct for biases in repertoire disease classification. We evaluate AIRIVA on both synthetic and real world immune repertoire datasets, as described below.

% In this section, our goal is to build AIRIVA models able to simulate wet-lab experiments such as exposure to one or multiple antigens. We empirically demonstrate that: i) AIRIVA is able to generate unbiased in-silico repertoires by correcting for undesired effects, and ii) AIRIVA performs competitively against group comparison baselines in predicting antigen-specific TCRs.

\subsection{Disentangling factors in variation in synthetic data}

In order to establish a proof of concept for the use of AIRIVA to disentangle factors of variation in TCR repertoire data, we first consider a fully synthetic dataset in which the underlying data generating process is perfectly known. We simulate such a dataset as follows...

\subsection{Identifying disease and vaccine-specific TCRs in COVID-19}
We evaluate AIRIVA in the context of SARS-CoV-2 (COVID-19) infection and vaccination, a data-rich setting for which the underlying biology is reasonably well-understood. The viral envelope of SARS-CoV-2 is made up of three proteins: the membrane protein, the envelope protein, and the spike protein (Figure~\ref{fig:covid_virus}). The spike protein is believed to be responsible for binding to host cells and initiating viral infection, and has therefore been the target of vaccine development. During natural infection, we expect to see expansion of TCRs associated with any one of these proteins, while in the case of vaccination with Johnson \& Johnson, AstraZeneca, Pfizer, or Moderna SARS-CoV-2 vaccines, we should only observe expansion of TCRs binding the spike protein. In the following experiment we aim to disentangle spike protein-specific TCRs from those TCRs associated with non-spike proteins.
% Figure~\ref{fig:virus_labels} shows the virus structure and label specification.

Our COVID-19 dataset comprises immune repertoires from a total of 7152 individuals in the training set and 5131 in the holdout set. Of those in the training cohort, 1954 have been positively diagnosed with a natural COVID-19 infection, 477 are healthy controls that have been vaccinated, and the remaining 5198 are unvaccinated healthy controls. Of those in the holdout cohort, 525 are PCR-positive for COVID-19, 400 have been fully vaccinated with one of the previously mentioned COVID-19 vaccines and have not had previous COVID-19 infection, 4606 are unvaccinated controls sampled prior to to the COVID-19 pandemic (December 2020), and the remaining 100 are vaccinated individuals that are PCR-positive for COVID-19.
We use disease and vaccination status to construct labels for \emph{non-spike} and \emph{spike} antigen exposure, as follows (Figure~\ref{fig:labels_def}): those samples with natural infection are labeled positive for both spike and nonspike antigens, $y_\text{infected} = [1,1]$. Healthy vaccinated samples are labelled as positive for the spike antigen but negative for nonspike antigens, $y_\text{vaccinated} = [0,1]$, while healthy unvaccinated samples are labelled negative for both, $y_\text{control} = [0,0]$. Note that we cannot observe repertoires exposed to nonspike antigens only.
% We use disease and vaccination status to construct labels  for "\textit{exposure to the spike protein}" (positive for both those in the vaccinated group, and those who are COVID-positive, that is, with natural infection) and "\textit{exposure to non-spike proteins}" (only those with natural infection). We will denote these two labels as \textit{spike} and \textit{non-spike} moving forward.
%Train
%Num vaccinated: 477/7152
%Num cases: 1954/7152
%Num controls: 5198/7152
% Holdout
%Num vaccinated: 400/5131
%Num cases: 525/5131
%Num controls: 4606/5131


% , due to the mismatch in depth of cases vs controls, that we wish to correct for.
% We also rely on HLA information in Section~\ref{sec:result_hla}.

\begin{figure}[]
	\centering
	%\includegraphics[width=\linewidth]{diagrams/intro_airiva.png}
	%\includegraphics[width=3cm]{example-image-c}
	
	\begin{subfigure}{0.45\linewidth}
		\includegraphics[width=1.0\linewidth]{figures/intro/covid_virus}
		\caption{SARS-CoV-2 structure}
		\label{fig:covid_virus}
	\end{subfigure}
	\begin{subfigure}{0.45\linewidth}
		\includegraphics[width=\textwidth]{figures/intro/covid_virus_labels}
		%\includegraphics[width=\textwidth]{figures/latent_space_vaccines2.png}
		\caption{AIRIVA label definition}
		\label{fig:labels_def}
	\end{subfigure}
	\caption{Disentangling disease-specific TCRs in COVID
	}
	\label{fig:virus_labels}
\end{figure}

\paragraph{Training}
We take as input to our model the counts of the $k$ most significant TCRs with respect to both spike and nonspike labels, based on $p$-values from the Fisher's exact test (FET).
Additionally, for each repertoire we have access to metadata such as sequencing depth, age, or inferred HLA status. In all the following experiments, we provide a measure of depth as an additional label---specifically, a standardized measure of log total template count---as depth is often a source of bias in repertoire disease classification.

We train AIRIVA on the training cohort, which is further partitioned 80:20 into train and validation, by maximizing the ELBO in \eqref{eq:elbo}.
We perform model selection running Bayesian optimization to maximize AUCROC \citep{Swamidass2010} for repertoire-level disease prediction on the validation set, sweeping over a wide range of hyperparameters, including encoder/decoder architecture, number of residual latents, number of predictive latents for sequencing depth, and weights for the various terms in the ELBO. Full details are provided in the appendix.

% Move to appendix:
% : learning rate, number of residual latents, number of predictive latents for sequencing depth, encoder/decoder network architecture (number of hidden layers), batch size, weights of each term in the ELBO, dropout probability, and L1/L2 regularization of encoder. See the Appendix for further details. For interpretability, we restrict the regressors of binary labels to be linear, such that any complex feature transformation occurs in the encoder.
%  We also implement softmax annealing in the variance of the reparametrization trick, which can be interpreted as sampling from a surrogate deterministic version of the posterior $\tilde{q}(z|x)$ with variance increasing with the number of iterations until it matches the variance of the original posterior ${q}(z|x)$.
%  We launch 20 agents in parallel, each of which executes 20 sequential runs for 2000 epochs.
%  We also consider pre-training followed by fine-tuning of some hyperparameters (L1 regularization, learning rate, batch size and weight of each term in the objective function) by launching 10 more agents with warm initialization to the best AIRIVA model from the first round of experiments.
%
% Having a two-step schedule in the tuning of loss term coefficients was helpful, favouring models that predict repertoire labels with high-accuracy first, after which we increase the weight of other terms in the objective function, i.e., the KL divergence and the reconstruction loss.
% Before training AIRIVA, we conduct a TCR selection preprocessing step to select a smaller subset of TCRs as input to the model using Fisher Exact Test with respect to each binary label. We report results for AIRIVA models trained on the union of 200 TCRs per label kept in the preprocessing step using per-label FET selection for the spike and non-spike label.

\paragraph{Evaluation with MIRA data} In addition to repertoire-level labelled data, we have access to `ground truth' labels on spike/nonspike TCR associations in the form of MIRA data, which forms the basis of our model evaluation. We have 422,933 MIRA hits for spike, and 1,238,238 for nonspike, of which 19,006 MIRA hits for spike and 50,050 for nonspike appear in at least 10\% of the covid-positive cases in the repertoire data. We use these 69,056 MIRA hits to assess the quality of learnt TCR-antigen associations from AIRIVA, and compare against baseline approaches.

%We compare each of these scores to average treatment effects per TCR from AIRIVA, and for each of these scores,
Specifically, given per-TCR scores for spike and non-spike antigen specificity, we can visualize these we these scores in scatterplot and quantify the correlation between spike and non-spike scores as measured by $R^2$ score; if these factors are perfectly disentangled, correlation should be zero.
We also evaluate classification performance against ground-truth from the wetlab based on MIRA hits (based on AUROC and sensitivity at 99\% specificity) for each score (e.g., for a spike score, spike MIRA hits are class 1, and non-spike MIRA hits are class 0).

% MEL: todo, rewrite by unifying explanation of FET-based scores and ATEs.
% a) describe each type of score
% b) describe groups for comparison
\paragraph{Benchmarks.}  Let $\mathcal{V}$, $\mathcal{C}^{+}$, and $\mathcal{H}$ refer to the set of TCR count repertoires for vaccinated, COVID-19-positive and healthy individuals respectively. We consider two baseline strategies for TCR-selection. Mean group difference scores and FET-based scores.
%
Mean group difference scores estimate the effect of spike and non-spike antigen exposure on each TCR by computing the difference in expectation of TCR counts between different groups of interest. In contrast, FET-based scores compares a case and control population using the Fisher Exact Test.
%
 Let $s_(g_1 , g_2)$ denote the strategy to compare two groups of repertoires $g_1$ and $g_2$. We consider two baseline strategies to compute the effect of exposure to spike and non-spike proteins on each TCR: the \textit{naive approach} and \textit{matched approach}. The naive approach compares the following groups:
	\begin{eqnarray}
		\delta_{\text{spike}} & = & s(\mathcal{C}^{+} \cup \mathcal{V}, \mathcal{H}) \\ %\mathbb{E}_{x \sim \mathcal{C}^{+} \cup \mathcal{V}}[x] - \mathbb{E}_{x \sim \mathcal{H}}[x] \\
		\delta_{\text{non-spike}} & = & s(\mathcal{C}^{+}, \mathcal{V}\cup \mathcal{H}),%\mathbb{E}_{x \sim \mathcal{C}^{+}}[x] - \mathbb{E}_{x \sim \mathcal{V}\cup \mathcal{H}}[x]
	\end{eqnarray}
where $\delta_{\text{spike}}$ and $\delta_{\text{non-spike}}$ quantify the effect of spike and non-spike antigen exposure per TCR based on the entire dataset and without accounting for any correlation between the antigen exposures.

In contrast, the matched approach aims to better match cases to controls by exploiting knowledge about the underlying causal mechanism. For the spike antigen, we compare vaccinated repertoires with healthy controls, ignoring the covid-positive as they have been exposed to both antigens. For the non-spike antigen, we compare the covid-positive groups against vaccinated repertoires. Let $\omega_{\text{spike}}$ and $\omega_{\text{non-spike}}$ correspond to antigen effects computed on dataset subsets to remove biased repertoires and better match cases against controls.
\begin{eqnarray}
	\omega_{\text{spike}} & = & s(\mathcal{V},\mathcal{H}) \\ %\mathbb{E}_{x \sim \mathcal{C}^{+} \cup \mathcal{V}}[x] - \mathbb{E}_{x \sim \mathcal{H}}[x] \\
	\omega_{\text{non-spike}} & = & s(\mathcal{C}^{+}, \mathcal{V}),%\mathbb{E}_{x \sim \mathcal{C}^{+}}[x] - \mathbb{E}_{x \sim \mathcal{V}\cup \mathcal{H}}[x]
\end{eqnarray}
%In the case of mean group differences,
%\begin{eqnarray}
%\omega_{\text{spike}} & = & \mathbb{E}_{x \sim \mathcal{V}}[x] - \mathbb{E}_{x \sim \mathcal{H}}[x] \\
%\omega_{\text{non-spike}} & = & \underbrace{\mathbb{E}_{x \sim \mathcal{C}^{+}}[x] - \mathbb{E}_{x \sim \mathcal{H}}[x]}_{\omega_{\text{spike+non-spike}}} - \left( \underbrace{\mathbb{E}_{x \sim \mathcal{V}}[x] - \mathbb{E}_{x \sim \mathcal{H}}[x]}_{\omega_{\text{spike}}} \right).
%\end{eqnarray}

\subsection{Robust HSV1 + HSV2 disease classification}
Finally, we evaluate repertoire classification with AIRIVA in another infectious disease setting, namely that of the highly prevalent HSV1 and HSV2 viruses. Infection can occur independently for each of these antigens, and also often co-occurs. This dataset comprises a small set of repertoires labelled according to HSV1/HSV2 status, together with a much larger cohort of unlabelled data known to have a high background rate of these viruses.



==> sections/problem.tex <==
\section{Problem Formulation}
We frame our results using the Neyman-Rubin potential outcomes framework
\citep{rubin2005causal}, as follows. We assume that for a unit with features
$x\in X$ , and an action (also known as treatment or intervention) $dss\in\{0,
    1\}$, there are two potential outcomes: $Y_0$ and $Y_1$. For each unit we only
observe one of the potential outcomes, according to treatment assignment: if $t
    = 0$ we observe $y = Y_0$, if $t = 1$, we observe $y = Y_1$; this is known as
the consistency assumption. For example, $x$ can denote the set of lab tests and
demographic factors of a diabetic patient, $t = 0$ denote the standard
medication for controlling blood sugar, $t = 1$ denotes a new medication, and
$Y_0$ and $Y_1$ indicate the patient’s blood sugar level if they were to be
given medications $t = 0$ and $t = 1$, respectively.

Throughout the paper, we assume that the following three
fundamental assumptions for treatment effect estimations
\citep{rosenbaum1983central} are satisfied: SUTVA, Unconfoundedness, overlap.

We consider an anti-causal binary prediction setting. Given $\numobs\in\N$
repertoires of $\numtcr$ recorded TCR counts, the goal is to predict whether a
repertoire was caused by a specific disease. We denote the matrix by

observational data, but interested in treatment effect

We make the following assumptions on the data set
\begin{itemize}
    % \item $\numobs$ - number of observations/persons \item $\numtcr$ - number
    % of pre-selected T cells (after exact Fisher test) \item $\nummeta$ -
    % number of additional features \item $\tcrmtrx_b\in {\{0,
    % 1\}}^{\numobs\times\numtcr}$ -  indicates the existence of a significant
    % amount of a T cell for each person \begin{itemize} \item \unsure{sparse}
    % but high-dimensional binary matrix \item \unsure{possibly measured with
    % noise} \end{itemize}
    \item $\tcrmtrx\in \mathbb{N}^{\numobs\times\numtcr}$ -  reports the counts
          of T cells for each person
          \begin{itemize}
              \item has more signal than binaries
              \item in code \texttt{cr_counts}:= convergent recombination counts
              \item \unsure{sparse} but high-dimensional binary matrix
              \item \unsure{possibly measured with noise}
          \end{itemize}
    \item $\dssvctr\in\mathbb{R}^{\numobs}$ - binary vector that denotes whether
          the person once suffered under the disease \sahra{Would it be reasonable to
              consider the time point of the disease instead?}
    \item $\mtmtrx\in\mathbb{R}^{\numobs\times\nummeta}$ - real valued matrix of
          meta values (additional features like age, gender, ...)
          \begin{itemize}
              \item meta values are not reliable
              \item often missing
              \item not available at test time
              \item helpful for robustness at training time
          \end{itemize}
    \item $\chrt\in\mathbb{N}$ - index denoting the cohort ID of a person/data
          set
    \item $\conf\in\mathbb{R}^{\numobs\times\nummeta}$ - unknown real-valued
          matrix that denotes confounding factors
    \item $\hla\in\{0, 1\}^{\numobs\times\nummeta}$ - binary matrix that denotes
          HLA \sahra{is this measured with noise?}
          \begin{itemize}
              \item Sex and Age do not influence HLAs
              \item an individual-level confounding factor
              \item correlated with ethnicity \sahra{are there relationships to
                        other meta data (i.e. gender)?}
              \item sometimes constant in a cohort
              \item find most important HLAs by comparing the frequency of each
                    HLA for diagnosed and healthy patients
              \item does not change for a single individual over time
              \item HLAs are risk factors for the disease but people without
                    HLAs can get diagnosed as well
              \item \sahra{He also finds that patients with a \unsure{higher
                            depth (i.e. more positive TCR values?)} are less likely to have
                        MS?}
              \item \sahra{What does it mean to have 0 or 20 HLAs in DIVA?}
          \end{itemize}
\end{itemize}

Assumptions at test time
\begin{itemize}
    \item Prediction of $\dssvctr$ given $\tcrmtrx$ in a previously unseen
          domain $\chrt$
    \item We do not assume we have access to $\chrt$
    \item We do not have access to all meta-values
    \item We have access to the depth and entropy
    \item We may or may not have access to $\hla$
\end{itemize}

Desirable properties
\begin{itemize}
    \item Robustness/Stability \sahra{Do we want to measure stability by the
              maximum deviation in the accuracy metrics across subgroups like Max?}
    \item Explainability/Understanding
\end{itemize}

Casual relationships:
\begin{itemize}
    \item the number of total templates, also known as the depth of a repertoire
          influences the observed TCRs, but has no causal relationship to the disease
          variable
    \item
\end{itemize}

==> sections/results_real_world_feb.tex <==
% Summary CLAIMS

% AIRIVA can be used to learn a factorized latent space (clusters) that is interpretable (vaccine clusters) and can be used to generate repertoires with specified characteristics (spike/nonspike/cmv <-> bar plots, masked heatmaps? age <-> cd4/cd8? depth <-> counts?)
% TCR-antigen association based on counterfactuals given inputs from naive FET approaches performance of matched FET, evaluating on MIRA.
% "Debiasing" for both covid and hsv1/hsv2: disentangling antigens and inclusion of potential confounders (age, depth) as labels can improve disease classification performance (especially as number of input TCRs is increased? in low data regimes?) (retraining on discovered tcrs?)


In this section, we empirically demonstrate AIRIVA's capacity to disentangle disease-specific TCRs and generate in-silico TCR repertoires.
%We evaluate AIRIVA on both synthetic and real world immune repertoire datasets.
%First, we show that AIRIVA is able to estimate average treatment effects accurately in a controlled synthetic setting.
%by correcting for different data biases in controlled synthetic scenarios.
We study AIRIVA in the context of two infectious diseases: SARS-CoV-2 and Human Simplex Virus infection. 
%\TM{What seems to be missing is an experiment with HLAs.  Could this be applied to HSV? We could then argue that for the sarscov2 the spike/nonspike is more interesting problem, which we expect would imporve with HLAs, but makes the experiments too compicated for our goal of ATEs/mira.  Our immunomics description really should empahsize the role of HLA, but our experiments do not.}
 
%\TM{No description of training set up, model selection, hyperparameter choices.}
%We go on to validate learnt TCR associations from our model against experimentally-derived TCR-antigen associations.
%
% 's benefits in the context of two real-world datasets including repertoires of patients diagnosed with COVID-19, and HSV-1 and HSV-2. Finally, we use external wetlab data to validate the TCR hits that our model discovers.
%
%The following analyses show that: i) AIRIVA can learn an interpretable latent representation of the data, ii) we can simulate in-silico TCR repertoires with manipulable characteristics conditioned on provided labels, iii) we can generate meaningful counterfactuals of observed repertoires, and iv) we can estimate causal effects while mitigating underlying biases in the data.
%v) we can improve the quality of AIRIVA as a simulator by adding additional labels.
%
%\paragraph{Dataset description}

%In the following, we consider two real-world datasets corresponding to immune-repertoires of cases and controls for two sets of infectious diseases: 
% The first dataset comprises a set of repertoires labelled according to HSV-1/HSV-2 status, captured by two binary labels $y_\text{hsv1}$ and $y_\text{hsv2}$. The second dataset includes labels for SARS-CoV-2 (COVID-19) infection and vaccination status.
%, together with a much larger cohort of unlabelled data known to have a high background rate of these viruses.

\paragraph{HSV}
The Herpes Simplex Virus (HSV) is classified into two types: HSV-1 and HSV-2.
%The two viruses share approximately 80\% of their genome~\cite{greninger2018ultrasensitive}, and will therefore have partially overlapping antigen sets and corresponding TCRs, making it challenging to build a model which accurately disentangles their labels.
Infections for both are frequent in the population, with $\approx$ 67\% prevalence for HSV1 and $\approx$ 13\% prevalence for HSV2~\cite{james2020herpes}. Infection status for either virus is independent of the other and infections can co-occur. Here we build an AIRIVA model to disentangle the two labels. 
The dataset comprises a total of 1125 repertoires in the training set, and 289 in the test set.
In addition to $\yvs_\text{hsv1}$ and $\yvs_\text{hsv2}$, we provide depth as an additional label $\yvs_\text{depth}$---a standardized measure of log total template count---as depth is often a source of bias in repertoire disease classification. Thus, we posit $\yv = \{\yvs_\text{hsv1}, \yvs_\text{hsv2}, \yvs_\text{depth}\}$. %Full details of the datasets are available in the Appendix.

\paragraph{SARS-CoV-2 (COVID-19)}
This dataset consists of repertoires labeled by SARS-CoV-2 (COVID-19) infection and vaccination status, with 7152 samples in the training set and 5131 in the test set.
%
The viral envelope of SARS-CoV-2 is made up of three proteins: the membrane protein, the envelope protein, and the spike protein. The spike protein is believed to be responsible for binding to host cells and initiating viral infection, and has therefore been the target of vaccine development. During natural infection, we expect to see expansion of TCRs associated with any one of these proteins, while in the case of vaccination\footnote{We consider viral vector vaccines AZD1222 (Oxford-AstraZeneca) and Ad26.COV2.S (Johnson \& Johnson), as well as mRNA vaccines BNT162b2 (Pfizer) and mRNA-1273 (Moderna).} we should only observe expansion of TCRs binding the spike protein. We thus posit $\yv = \{\yvs_\text{ns}, \yvs_\text{s}, \yvs_\text{depth}\}$, where $\yvs_{ns}$ and $\yvs_s$ refer to exposure to the nonspike and spike proteins respectively, and $\yvs_\text{depth}$ refers to sequencing depth as described above.

%
%{\color{red} TODO: say something about how train and holdout are chosen? Are these i.i.d or not?}

\paragraph{Experimental Setup}
%Given the high-complexity of the considered TCR repertoire,
We conduct a pre-processing step using a Fisher's Exact Test (FET) with respect to each binary label and feed the union of these FET-filtered TCR subsets to AIRIVA. Although alternative approaches can be considered, FET-based TCR selection has been shown to work well to generate a higher signal-to-noise set of TCRs. 
%
To further validate the capacity of AIRIVA to disentangle unrelated signal, in the case of COVID-19 experiments, we also include a subset of FET-selected TCRs known to be associated with cytalomegalovirus (CMV), a virus with approx. 50\% prevalence in the population~\citep{Staras2006} that we know to be unrelated to the binary labels. We train our model with 612 input TCRs in total for COVID-19, and 325 TCRs for HSV. See the Appendix for full details.

\paragraph{Model Training and Selection}  
We train AIRIVA by maximizing the regularized ELBO in Eq.~\eqref{eq:elbo}. We conduct a random sweep for hyperparameter search, and perform model selection in two steps: 
i) rank runs by highest average area under concentrated ROC (AUCROC)~\cite{Swamidass2010} for repertoire-level prediction of labels on the validation set; such ranking by AUCROC enable us to identify a reduced set of top candidate models; 
ii) select the best run as the one with better qualitative latent space (in terms of clear separation between clusters and matching between the prior and posterior).

\paragraph{Validation with ground-truth MIRA}\label{sec:mira}
In addition to repertoire-level labels, in the case of COVID-19 we have access to external in-vitro labels on spike and nonspike TCR associations from MIRA (\textbf{M}ultiplexed \textbf{I}dentification of T cell \textbf{R}eceptor \textbf{A}ntigen specificity) experiments~\cite{klinger2015multiplex}.
The data comprises over 400k experimentally-derived TCR-antigen binding pairs for the spike protein, and 1.2M for nonspike proteins. Of these, 75 spike and 105 nonspike associated TCRs appear in our set of 612 TCRs from FET used as input to AIRIVA.
% We have 422,933 MIRA hits for spike, and 1,238,238 for nonspike, of which 19,006 MIRA hits for spike and 50,050 for nonspike appear in at least 10\% of the covid-positive cases in the repertoire data. 
We use these spike and nonspike associated TCRs from MIRA to assess the quality of learned TCR-label associations from AIRIVA.
%, and compare against group mean differences between cases and controls.

\begin{figure*}[]
	\centering
	\begin{subfigure}{0.45\textwidth}
		%\includegraphics[width=\textwidth]{figures/latent_space/fig1a_annotated}
        %\includegraphics[width=\textwidth]{figures/covid/latent_covid_best.png}
        \includegraphics[width=\textwidth]{figures/final/best_run/latent_holdout.png}
        \caption{Latent space stratified by subgroup}
        \label{fig:latent_space_COVID}
	\end{subfigure}
        \hspace{0.5cm}
        \begin{subfigure}{0.43\textwidth}
            \includegraphics[width=\textwidth]{figures/final/best_run/latent_space_vaccine3}
            \includegraphics[width=\textwidth]{figures/final/best_run/vaccine1.png}
            \caption{Latent space stratified by vaccine type}
            \label{fig:vaccine_latent_space}
        \end{subfigure}
	\caption{\textbf{Latent space for SARS-CoV-2}. Each point corresponds to one sample $\sz$ from the posterior $q(\zv|\xv)$ in holdout. On the sides, we show the marginal posteriors as continuous lines, and predictive priors as dashed lines. (a) Predictive priors $p(\zv_y|\yv)$ for each combination of labels are represented as ellipses, each circle denoting one standard deviation. (b) Posterior samples for vaccinated subgroups (coloured), ellipses here correspond to the fit of 2D multivariate Gaussians; samples for other subgroups are shown in grey.}
	\label{fig:latent_space_COVID}
\end{figure*}

% \section{Results}

\subsection{Disentangled Latent Representation}

%Turning now to real repertoire counts data, we show that AIRIVA can be used to learn a factorized latent space that is interpretable and manipulable, i.e. can be used to generate repertoires conditioned on specific characteristics, as well as counterfactuals.
% (spike/nonspike/cmv <-> bar plots, masked heatmaps? age <-> cd4/cd8? depth <-> counts?)
Visualizing latents for AIRIVA trained on the COVID-19 dataset, we can see that the model is able to learn a factorized, interpretable latent space, with predictive latents corresponding to the provided labels. 
Figure~\ref{fig:latent_space_COVID} shows posterior samples from $q(\zv_y|\xv)$ for holdout data and the exact learned prior predictive distributions $p(\zv_y|\yv)$ in the latent subspace ($\zv_\text{nonspike}$, $\zv_\text{spike}$), stratified by subgroups. Note that one of the label groups, that correspond to ``\textit{nonspike only}'' exposure, is never observed in the real-world since both spike and nonspike co-occur during infection. As expected, the vaccinated subgroup exhibits only spike signal (variability along the top-left corner), whereas COVID-positive cases either with and without vaccination show exposure to both spike and nonspike antigens (top-right corner). Appendix Figure~\ref{fig:latent_space_hsv12}, shows a similar latent space representation for AIRIVA trained on HSV. Again, we see changes in HSV-1/HSV-2 status of repertoires along the corresponding predictive latent axes.

Such a structure latent space can be interpreted to provide biological insights into observed immune response. 
%\TM{Such as structure latent space can be interpreted as XYZ to provide ABC}
Figure~\ref{fig:vaccine_latent_space} shows the posterior samples of the vaccinated repertoires in holdout stratified by vaccine type; samples from other subgroups are plotted in grey. We show a 2D-Gaussian fit (each ellipse represents one standard deviation)
%\TM{stdev details in caption, what is the take away message in text?}
to the posterior distribution of each vaccine type. Interestingly, our model suggests that repertoires that were administered the AstraZeneca viral vector AZD1222 vaccine exhibit lower spike T-cell response compared to mRNA vaccines from Johnson \& Johnson, Pfizer or Moderna which is consistent with findings in the literature \citep{Schmidt2021,Prendecki2021,Marking2022}.
%AstraZeneca vaccines exhibit less spike signal, whereas Pfizer and Moderna vaccines yield the highest response to the spike protein, which is consistent with the literature.

%shows that when stratified by vaccination type, repertoires that were administered the viral vector AZD1222 vaccine exhibit lower spike T-cell response compared to mRNA vaccines, which is consistent with findings in the literature \citep{Schmidt2021,Prendecki2021,Marking2022}.
%






%\TM{Move CG and CFG to methods/ treatment effects section and refer to that here.  Here keep only the results on the datasets and their comparision to baselines group mean diff etc}
\subsection{Conditional Generation}

We can use this factorized latent space to generate in-silico repertoires conditioned on specific label values. We do so by sampling the latent representation $\sz$ given the labels $\sy$, and in turn the TCR counts $\sx$ given $\sz$, as stated by Equation~\eqref{eq:generative_process}. 
This can be useful, for example, in simulating repertoires from subgroups or label combinations with lower prevalence in observational data, in order to curate a more balanced dataset for downstream tasks.

\begin{figure*}[h!]
\centering
\begin{minipage}[t]{0.6\textwidth}
\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=\linewidth]{figures/final/best_run/mira_counts_cond_gen.png}
    % \includegraphics[width=\linewidth]
    % {figures/final/airiva_mira_counts.png}
    \caption{Average number of TCR counts in the input space}
    \label{fig:binary}
\end{subfigure}
\vspace{-0.5em}
\begin{subfigure}[t]{\linewidth}
    %\includegraphics[width=\linewidth]{figures/final/heatmap_decoder2.png}
    \includegraphics[width=\linewidth]{figures/final/best_run/decoder_heatmap.png}
    \caption{Average decoder Poisson rate in the latent space}
    \label{fig:decoder_heatmap}
\end{subfigure}
\end{minipage}
\hfill
\begin{subfigure}[!t]{0.38\linewidth}
    %\includegraphics[width=\linewidth]{figures/final/depth_intervention.png}
    \includegraphics[width=\linewidth]{figures/final/best_run/cond_gen_depth_no_fliers.png}
	\caption{TCR counts when intervening on depth}
	\label{fig:effect_interven_depth}
\end{subfigure}
\caption{\textbf{Conditional generation with AIRIVA}. (a) Mean activation per TCR in input space (in decreasing order), where activation corresponds to the average of TCR counts across repertoires plus one standard deviation. 
%\TM{Not enough description to undertand the figure.  Needs to be crystal clear in text or here.  What is the take awya?}
(b) Decoder Poisson rate averaged across different types of TCR mapped to the latent space.
(c) Depth distributions on factual and in-silico data.
%See corresponding plots for factual data in Appendix.
 }
\end{figure*}

Taking AIRIVA trained on the COVID-19 dataset, we evaluate whether conditionally generated repertoires have the properties we expect.\footnote{As a reminder, we only have access to TCR annotations for the COVID-19 dataset.}
% One way to validate if AIRIVA is a good simulator of our data is to generate repertoires conditioned on the labels, and check whether such repertoires have the expected properties. 
In particular, repertoires of vaccinated and COVID-positive individuals should exhibit higher counts of spike specific TCRs, while nonspike specific TCRs should only activate for COVID-positive ones. %We generate repertoires conditionally by intervening on the spike and nonspike labels, and for an average mean depth.
Figure~\ref{fig:binary} shows the average activation per TCR, defined as the average TCR count plus one standard deviation, when generating repertoires conditioned on different values for spike and nonspike labels. In each case, the value of the depth label is set to the median depth in the training data.

TCRs are stratified according to their spike/nonspike annotations from MIRA (described in Subsection~\ref{sec:mira}), as well as CMV association. As expected, generating ``vaccinated" repertoires (with spike only) results in increased activation of spike MIRA hits, while conditionally generating  natural infections (with positive spike and nonspike labels) shows increased activations in both spike and nonspike MIRA TCRs. On the other hand, activation of CMV-associated sequences remains negligible across all label groups, which brings empirical evidence that AIRIVA is able to keep other structural signal separated ---captured by the residual latent subspace $\sz_{\epsilonv}$--- from the  latent subspace of interest, i.e., spike/nonspike signal.
%
%These findings are robust to different values of sequencing depth, as shown in the Appendix.

Figure~\ref{fig:decoder_heatmap} illustrates the Poisson rates splitted by the same TCR subsets when sweeping over coordinates in the latent subspace ($\sz_\text{nonspike}$, $\sz_\text{spike}$). We can see that, for spike MIRA hits, the decoder is able to learn decision boundaries that are orthogonal to $\sz_\text{spike}$. For the nonspike TCRs however, we find that the decision boundary is warped in the lower right nonspike-only region of the space. This is expected, as the region for which we have no data in observed repertoires and the decoder has no information to learn an orthogonal boundary without further inductive biases in the out-of-distribution region. The activation for CMV annotations remain mostly inactive in the latent spike/nonspike subspace, highlighting AIRIVA's capacity to disentangle different underlying signals.

%\TM{Not enough info for reader} 
Finally, Figure~\ref{fig:effect_interven_depth} compares the distribution of total sum of TCR counts for conditionally generated in-silico repertoires against the empirical distribution when stratifying by depth. Although the in-silico repertoires tend to exhibit a higher number of outliers due to the assumed Poisson distribution, the marginal distribution of in-silico repertoires follows the same trend than the empirical one, enabling us to control depth in a realistic manner.

% \begin{figure}[h!]
% 	\centering
% 	%\includegraphics[width=\linewidth]{figures/final/depth_intervention.png}
%  \includegraphics[width=\linewidth]{figures/final/best_run/cond_gen_depth_no_fliers.png}
% 	\caption{Conditional generation by intervening on depth. (left) factual data; (right) in-silico data, conditionally generated repertoires with same marginal depth distribution.} 
% 	\label{fig:effect_interven_depth}
% \end{figure}

\begin{figure*}[h!]
	\centering
	\begin{subfigure}{0.45\textwidth}
		%\includegraphics[width=\linewidth]{figures/covid/coutnerfactuals_best.png}
        \includegraphics[width=\linewidth]{figures/final/best_run/counterfactuals_all_stochastic1b.png}
		\caption{Posterior samples $\sz \sim q(\zv|\xv)$ for COVID-19}
	\end{subfigure}
        \hfill
	\begin{subfigure}{0.53\textwidth}
		\includegraphics[width=\linewidth]{figures/final/best_run/counterfactuals_all_stochastic2b.png}
		\caption{Posterior predictive $q(\yv|\xv)$ for COVID-19}
	\end{subfigure}
 
 \vspace{0.3cm}
 
 \begin{subfigure}{0.49\textwidth}
        \includegraphics[width=\linewidth]{figures/hsv12/best_run/counterfactuals1.png}
	\caption{Posterior samples $\sz \sim q(\zv|\xv)$ for HSV}
	\end{subfigure}
        \hfill
	\begin{subfigure}{0.49\textwidth}
		\includegraphics[width=\linewidth]{figures/hsv12/best_run/counterfactuals2.png}
		\caption{Posterior predictive $q(\yv|\xv)$ for HSV}
	\end{subfigure}
	\caption{\textbf{Counterfactual generation with AIRIVA}. (left) Latent representation $\sz \sim q(\zv|\xv)$ for factual data (first column) and counterfactual data (other columns) stratified by subgroups. (right) Posterior predictive distribution $q(\yv|\xv)$ for factual (first column) and counterfactual data (columns 2-5) stratified by subgroups. The labels assignment is: control = [0 0], hsv2 [0 1], hsv1 [1 0], hsv1+hsv2 [1 1].
    %The ``nonspike only'' subgroup can never be observed in reality. %Similar plots for HSV dataset can be found in Figure~\ref{fig:counterfactuals_hsv} of the Appendix.
	}
	\label{fig:counterfactuals}
\end{figure*}

\begin{figure*}[h!]
	\centering
 %\includegraphics[width=\linewidth]{figures/final/mira_covid.png}
 %\includegraphics[width=\linewidth]{figures/final/ates.png}
        \begin{subfigure}{0.24\textwidth}
		\includegraphics[width=\textwidth]{figures/final/best_run/ates/ate_naive.png}
		\caption{Naive cases to controls}
		\label{fig:ate_naive}
	\end{subfigure}
	\begin{subfigure}{0.23\textwidth}
		%\includegraphics[width=\textwidth]{figures/GMD_all_independent}
      \includegraphics[width=\textwidth]{figures/final/best_run/ates/ate_matched.png}
		\caption{Matched cases to controls}
		\label{fig:ate_matched}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.24\textwidth}
		%\includegraphics[width=\textwidth]{figures/mean_diff_oracle}
        \includegraphics[width=\textwidth]{figures/final/best_run/ates/ate_cond_gen.png}
		\caption{AIRIVA cond. generation}
		\label{fig:ate_cond}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.24\textwidth}
		%\includegraphics[width=\textwidth]{figures/ate_counterfactual_AIRIVA}
        \includegraphics[width=\textwidth]{figures/final/best_run/ates/ate_ctf_10_00.png}
		\caption{AIRIVA counterfactuals}
		\label{fig:ate_cf}
	\end{subfigure}
	\caption{\textbf{Estimation of conditional average treatment effects for COVID-19.} by (a) Naive approach: splitting all available individuals into cases and controls for each positive label, regardless of any unobserved confounder, (b) selecting subsets in the dataset to match marginal label distributions between cases and controls, (c-d) using AIRIVA to impute the potential outcomes and estimate average treatment effects via (c) conditional generation or (d) counterfactuals. On top of each Figure We report the Spearman correlation between ATEs (closer to zero, the better)}
 %In this example, we estimate the effect of the spike antigen by taking all vaccinated individuals, and compute their corresponding counterfactual of removing the effect of vaccine.}
	\label{fig:figure_ATEs}
\end{figure*}


\subsection{Counterfactual Generation}

%The model, that by itself is a useful tool to interpret the data, also provides a meachanism to generate realistic counterfactuals. These synthetically generated data allows us to use the model as a \emph{data driven simulator for immunomics}.

Next, we assess AIRIVA's capacity to generate counterfactuals by intervening on the labels, as described in Section~\ref{sec:counterfactuals}. Figure~\ref{fig:counterfactuals}a shows the latent space representation of the observed data (first column), and counterfactuals (other columns) transformed from one subgroup to another. Figure~\ref{fig:counterfactuals}b shows the corresponding posterior predictive distribution $q(\yv|\xv) = \int q(\yv|\zv)q(\zv|\xv)d\zv$ for factuals and counterfactuals.
%
Both figures show that we can generate counterfactuals by manipulating specific labels. We note that the last column corresponds to a repertoire subgroup that can never been seen in reality: these are out-of-distribution counterfactuals. Interestingly, although AIRIVA is not supposed to handle those correctly without further inductive biases, it manages to learn the right direction of variation in the latent space.


 \subsection{Identifying Label-Specific TCRs}

Ultimately, our goal is to be able to use AIRIVA to identify TCRs that respond to the disease or label of interest.
In this section, we aim to estimate the effect of exposure to a given antigen on individual TCRs, which we will call the \textit{treatment effect} thereof. In the case of COVID-19, we are interested in the treatment effect of spike and nonspike proteins on the TCR counts repertoire.
%, and the exposure to HSV1 and HSV2 virus in the case of Human Simplex Virus.
We know from the underlying biology that each individual TCR should bind to either of these proteins but not to both simultaneously: we thus expect the treatment effect for spike and nonspike to be uncorrelated. 
%In the following, we compare different strategies for average treatment effect estimation of a given label conditioned on the other labels, using ground-truth annotations from MIRA, as described in Section~\ref{sec:mira}.
%
Disentangling this signal is key to differentiating natural infection, where repertoires are exposed to both spike and nonspike proteins, from vaccinated individuals exhibiting only spike response, as sketched in Appendix Figure~\ref{fig:covid_data_structure}, but is challenging in practice.
%(\TM{Evidence?  Why?}.

% Identifying which TCR binds to which protein is a challenging task given that both proteins co-occur in COVID natural infections, as shown in Fig.~\ref{fig:figure_ATEs}a.
%positive for either of these, but not simultaneously. We can then validate AIRIVA capacity to estimate ATEs by measuring correlation between ATEs.
%
% Identifying which TCR binds to which protein is a challenging task given that both proteins co-occur in COVID natural infections, as shown in Fig.~\ref{fig:figure_ATEs}a.
To illustrate this, let us split the observed population into cases and controls naively according to each binary label, and estimate the average treatment effect (ATE) empirically via difference of group expectations in TCR counts. We can see from Figure~\ref{fig:ate_naive} that this approach suffers from significant confounding due to the COVID-19 positive group and is unable to distinguish spike and nonspike TCRs from MIRA, yielding biased estimations of the conditional ATEs.

\begin{figure*}[h!]
	\centering
 %\includegraphics[width=\linewidth]{figures/final/mira_covid.png}
 %\includegraphics[width=\linewidth]{figures/final/ates.png}
        \begin{subfigure}{0.24\textwidth}
		\includegraphics[width=\textwidth]{figures/final/hsv/naive.png}
		\caption{Naive cases to controls}
		\label{fig:ate_naive_hsv}
	\end{subfigure}
	\begin{subfigure}{0.23\textwidth}
      \includegraphics[width=\textwidth]{figures/final/hsv/matched.png}
		\caption{Matched cases to controls}
		\label{fig:ate_matched_hsv}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.24\textwidth}
		%\includegraphics[width=\textwidth]{figures/mean_diff_oracle}
        \includegraphics[width=\textwidth]{figures/final/hsv/airiva_cond.png}
		\caption{AIRIVA cond. generation}
		\label{fig:ate_cond_hsv}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.24\textwidth}
		%\includegraphics[width=\textwidth]{figures/ate_counterfactual_AIRIVA}
        \includegraphics[width=\textwidth]{figures/final/hsv/airiva_ctf.png}
		\caption{AIRIVA counterfactuals}
		\label{fig:ate_cf_hsv}
	\end{subfigure}
	\caption{\textbf{Estimation of conditional average treatment effects for HSV.} by (a) Naive approach: splitting all available individuals into cases and controls for each positive label, regardless of any unobserved confounder, (b) selecting subsets in the dataset to match marginal label distributions between cases and controls, (c-d) using AIRIVA to impute the potential outcomes and estimate average treatment effects via (c) conditional generation or (d) counterfactuals. On top of each figure we report the Spearman correlation between ATEs (the closer to zero, the better)}
 %In this example, we estimate the effect of the spike antigen by taking all vaccinated individuals, and compute their corresponding counterfactual of removing the effect of vaccine.}
	\label{fig:figure_ATEs_hsv}
\end{figure*}

One way to address such known sources of confounding is to better match cases and controls by excluding samples responsible for those undesired effects. Concretely, given our understanding of the subgroups in this data, we can instead estimate per-TCR ATEs for nonspike by comparing natural infection against vaccinated repertoires only (dropping controls), and the ATEs for spike by comparing vaccinated against healthy repertoires (dropping samples with natural infection), as shown in Figure~\ref{fig:ate_matched}.
%
However, we can see that this introduces new biases in the ATE estimation: while we are better positioned to distinguish spike and nonspike MIRA hits (MIRA hits are easily separable), we now observe a negative correlation between spike and nonspike conditional ATEs. In practice, it is impossible to account for all possible confounders to create balanced case and control populations, particularly in data-limited settings.
% Dropping samples that contaminate the effect estimations in undesirable ways is sample inefficient and time-consuming---domain experts need to explore and understand data properties.



Instead, we can use AIRIVA to either conditionally generate matched populations in-silico (Figure~\ref{fig:ate_cond}), or to estimate counterfactuals, and handle biases without any manual matching. Figure~\ref{fig:ate_cf} shows the estimated conditional ATEs when generating counterfactuals as discussed in Section~\ref{sec:counterfactuals}. In particular, for any observed sample, we impute the unobserved potential outcome by generating its corresponding counterfactual following the procedure described in Algorithm~\ref{algorithm1}. We then compute the averaged treatment effect of each protein exposure as the difference in potential outcomes, conditioned on switching off other binary labels. 

% for each subgroup in the dataset, we map observed repertoires to nonspike only, as in the last column of figure, to get our set of nonspike counterfactual outcomes. for the rest of controls
% \begin{equation}
% \text{ATE}_{cf} =  ... % (X(sick -> ns) + X(vaccine --> ns) + X(control --> ns)) - (X(sick -> ns) + X(vaccine --> ns) + X(control --> ns)) - (X_control + X(sick --> control) + (X_vaccine --> control))
% % \eq \mathbb{E}_i\left[ \tau_i \right] = \mathbb{E}_i\left[ X_i(0) - X_i(Y) \right].
% \end{equation}
% Following the Neyman-Rubin potential outcomes framework~\cite(rubin2005causal), each individual $i$ has two potential outcomes: let $X_i(0)$ be the TCR counts for a healthy individual, and $X_i(1)$ the TCR counts if the individual has been exposed to the disease antigen in question. Formally, the observed TCR counts for an individual (or factual data) can be written as $x_i \defeq X_i(0) \cdot (1-y_i) + X_i(1)\cdot y_i$. For each individual, the effect of a given label $y_i$ on the repertoire is captured by the \textit{individual treatment effect}, defined as $\tau_i = X_i(1) - X_i(0)$. To quantify the expected causal effect of a given label on the TCR counts, we are interested in the \textit{average treatment effect} (ATE), defined as:
% \begin{equation}
% \text{ATE} \defeq \mathbb{E}_i\left[ \tau_i \right] = \mathbb{E}_i\left[ X_i(0) - X_i(Y) \right].
% \end{equation}
The conditional ATEs estimated using AIRIVA are fully de-correlated for spike and nonspike TCRs from MIRA, providing empirical evidence that AIRIVA learned meaningful disentangled factors that can be manipulated to impute unobserved potential outcomes
%
Interestingly, nonspike conditional ATEs would be impossible to compute directly using observational data, as ``nonspike only'' samples are never seen in reality.
%
Figure~\ref{fig:figure_ATEs_hsv} shows the estimated conditional ATEs for HSV-1 and HSV-2 based on naive and matched group mean differences or imputing potential outcomes using AIRIVA. While we do not have access to ground truth TCR associations, we can see that AIRIVA-generated conditional ATEs are largely decorrelated for HSV-1 and HSV-2, behaving similarly to the matched group mean difference approach. This demonstrates that AIRIVA can be trained to capture meaningful disentangled signal, which can then be manipulated 
 by intervening on the binary labels.



% In the case of counterfactual ATEs, this is less clear; while we are able to recover TCRs with high ATE for HSV-2 only, much of the HSV-1 signal appears to correlate with HSV-2. This may be partly attributed to the similarity in the genome of HSV-1 and HSV-2; we expect that in this setting, a subset of TCRs may be specific to both disease antigens.
%% We can also assess the model's ability to retrieve relevant TCRs by evaluating disease classification performance at the repertoire level...
%
% To account for this, we can use a model such as AIRIVA to "clean" up the contamination by learning to decompose the signal (see Figure~\ref{fig:third}).


% sickness-> vaccine depth shift discussion: lymphopenia (+severity), t-cell fraction, assume fraction of t-cells are t-cells.  see Rachel's paper. 2) sample type -- cohort blood/pbmc/dna, time from infection.

 % unconfounded TCR classification based on estimation of per-TCR average treatment effects, where treatment refers to ``exposure to a given antigen''.
 % AIRIVA can identify antigen specific TCRs that are highly correlated in the observed repertoires (and thus, hard to disentangle)
 % Fig 1: Disentanglement of TCRs (key result of the paper, external validation with MIRA): effect size per TCR for spike (x-axis) and nonspike (y-axis) for a) FET-based scores (p values), b) observational ATEs, c) AIRIVA-based ATEs via conditional generation, d) AIRIVA-based ATEs via counterfactuals.

% \subsubsection{Treatment effect estimation with AIRIVA can disentangle antigen-specific TCRs}


% EXPLAIN: 
 %  when we have perfect controls and do not have confounders that bias the ATE (differences in expectations) or FET (assignments to case/controls).  If we have perfect assignments, to cases and controls, we do not need a model and the FET/empATE is sufficient.

 % To do the FETs above we needed to drop the healthy controls from the NS estimates and drop the covid+ from the S estimates.  Both contaminate the effect estimations in undesirable ways.  For NS estimation, the healthy controls overestimate Spike signal and for S estimation the Covid samples add NS noise.  Both of these effects are seen in the correlation plots we originally showed between the spike / nonspike neg-logp plots or group mean differences.

 % TED: we can compare the perfect FET/empATE results with our model based ATEs that use more data and importantly, contaminated labels.  Having a model such as AIRIVA "clean" up the contamination by learning to disentangle the signal.

 % \subsection{Handling bias in repertoire classification}
 % %AIRIVA can perform de-confounded multi-endpoint predictions at the repertoire level.
 % %AIRIVA can predict multiple repertoire labels of interest jointly (e.g., disease diagnostic, risk alleles) while accounting for undesired effects (e.g. depth).

 % In this Section, we show that AIRIVA can learn how to adjust for undesired effects such as sequencing depth while predicting for repertoire labels in a unified framework. This can be done by adding sequencing depth as an additional label to the model and using some dimensions of the latent space $z_{depth}$ to account for differences in the overall number of TCR counts in different repertoires. Intuitively, the latent subspace $z_{depth}$ corrects for different generation probability of TCRs (some sequences are more likely than others) before any antigen exposure, and equalizes repertoires of different depth.

 % Table~\ref{tab:per-group} shows the predictive performance of an AIRIVA model with and without depth as label. Adding such a depth label improves per-group predictive performance as measured by sensitivity at 99\% specificity, and reduces instability (range differences between groups of different depth).


%To recap, while the matching approach from Figure~\ref{fig:ate_matched} entail dropping samples to compare similar cases to controls, AIRIVA imputes the missing potential outcomes and uses all available data to estimate the conditional ATE effects.





























%  \subsection{Classification of HLA context-specific TCRs}\label{sec:result_hla}
%  % describe cluster assignments, experimental setup, etc @Niranjani

%  \paragraph{Fig} per-HLA conditional effect size per TCR for (a) spike (x-axis) and nonspike (y-axis) in A*(02/01):01 HLA  cluster, (b) not in this cluster, (c) Non spike ATEs in (y-axis) and out (x-axis) of cluster, (d) spike ATEs for the same. Ideally, what we want to see here is nonspike/spike MIRA hits respectively along each axis.

% \begin{figure}[]
% 	\centering
% 	\includegraphics[width=0.5\textwidth]{figures/per_hla}
% 	\caption{[PLACEHOLDER] (visual diagram with the paper TLDR/goals): a) ATEs for different HLAs and antigens (2D plots, some sort of pairplot, b) number of MIRA hits found in each group?)}
% 	\label{fig:hla}
% \end{figure}

% \subsection{(AIRIVA in-silico repertoires retain label information)}
% % in-silico generation of repertoires with downstream applications such as data augmentation, ATE/CATE estimation.
%
% Using in-silico AIRIVA-generated repertoires yield high predictive performance, comparable to real repertoires. Below some experiment ideas we could conduct to argue this point:
%
% Option 1. train an ESLG/EMLG model with only in-silico AIRIVA-generated repertoires. Do we obtain similar predictive performance as a model trained on observed repertoires?
%
% Option 2: suppose we have limited number of observed repertoires. We train an AIRIVA model with such reduced dataset, and then train an ESLG model with (observed + in-silico) repertoires. Can we improve predictive performance of ESLG? [Skeptical, because if we have reduced number of repertoires, that will impact the quality of the learned AIRIVA model].
%
% Option 3: train an AIRIVA model, and then generate a much smaller set of in-silico repertoires. The hope is that AIRIVA can learn to generate "unbiased" datasets, such that with same amount of data, in-silico repertoires exhibit a cleaner signal.

% \subsection{AIRIVA can generate realistic in-silico repertoires.}

% The characteristics of AIRIVA-generated TCR count repertoires are similar to the real repertoires (such as Fig. 5 from Davidsen et.al, 2019, see below, and note that this Figure was generated for a sequence model, but we should be able to plot similar statistics for TCR count repertoires).

% \paragraph{Fig} Statistics of interest for real and in-silico repertoires

% \subsection{AIRIVA can predict multiple repertoire labels robustly}
% %AIRIVA can perform de-confounded multi-endpoint predictions at the repertoire level.
% AIRIVA can predict multiple repertoire labels of interest jointly (e.g., disease diagnostic, risk alleles) while accounting for undesired effects (e.g. depth).
% AIRIVA exhibits similar predictive performance as logistic regression-based models. Performance measured in terms of sensitivity (if we can isolate a more meaningful set of TCRs (true spike and nonspike signal), then we should be able to achieve similar or even higher sensitivity in certain scenarios (especially with is distribution shift in input data, such as different cohort).
% \paragraph{Fig} ROC curves for best models (1st row = spike prediction task; 2nd row = nonspike prediction task), in each column, 2 baselines: ESLG, EMLG. Train and holdout curves.

% \begin{table}[h!]
% 	\begin{center}
% 		\begin{tabular}{c||c|c|c}
% 			\toprule
% 			%& \multicolumn{2}{c|}{LG-based models} & \multicolumn{2}{c}{AIRIVA} \\
% 			%\midrule %\cmidrule{1-2} \\
% 			Metric & Sensitivity@0.99 & AUCROC & FPR(vaccinated) \\
% 			\midrule
% 			ESLG & $0.6 \pm 0.01$ &  $0.6 \pm 0.01$ & $0.6 \pm 0.01$ \\
% 			EMLG & $0.6 \pm 0.01$ &  $0.6 \pm 0.01$ & $0.6 \pm 0.01$ \\
% 			\midrule
% 			AIRIVA & $0.6 \pm 0.01$ & $0.6 \pm 0.01$ & $0.6 \pm 0.01$ \\
% 			\bottomrule
% 		\end{tabular}
% 		\caption{Predictive performance with confidence intervals by bootstrapping predictions in holdout set.}
% 	\end{center}
% \end{table}

% \paragraph{Fig (?)} Robustness to depth (AIRIVA with and w/o explicit depth factor; comparision with E(M)LG, which does have explicit depth correction?)

% %In terms of sensitivity in some settings (if we can isolate a more meaningful set of TCRs (true spike and nonspike signal), then we should be able to achieve similar or even higher sensitivity in certain scenarios (especially when there is distribution shift in input data, such as different cohort).
% %
% %Fig 3: ROC curves for best models (1st row = spike prediction task; 2nd row = nonspike prediction task), in each column, 3 baselines. Train and holdout curves.
% %
% %Fig 4: Predictions stratified by cohort
% %
% %Table 2: Sensitivity@99.8 for each model and baseline with confidence intervals by bootstrapping predictions in holdout set, probably stratified by cohort?

% \subsection{AIRIVA can extract interpretable latent dimensions}
% %\subsection{Disentanglement of repertoires in the latent space}
% We now demonstrate that AIRIVA is able to learn interpretable human-concepts  that facilitate exploratory analysis. (...)
% The probabilitistic representation learned by AIRIVA can be used to draw important biological conclusions. For instance... Explain vaccine.

% AIRIVA can learn an interpretable latent representation where each dimension is an interpretable human-concept, facilitating qualitative exploration (metric: correlation of z-scores with actual labels + latent space)

% \paragraph{Fig} Latent space representation (samples from posterior + exact Gaussian priors on top (todo) - current figs as placeholder + per-vaccine exploration.

% %Interpretability: we learn a latent representation where each dimension (axis) is an interpretable human-concept, facilitating qualitative exploration by experts in the field. To illustrate this claim, we show exploration of vaccines in latent space.

% %Fig 6: a) posterior distribution in latent space, b) only vaccinated, coloring by vaccination type and by number of doses; c and d) same visualizations but for the multi-task feedforward NN baseline, I.e., 2-dim visualization of hidden layer.


% \subsection{AIRIVA enables deconfounded TCR classification}
% % unconfounded TCR classification based on estimation of per-TCR average treatment effects, where treatment refers to ``exposure to a given antigen''.
% % AIRIVA can identify label specific TCRs that are highly correlated in the observed repertoires (and thus, hard to disentangle)
% % Fig 1: Disentanglement of TCRs (key result of the paper, external validation with MIRA): effect size per TCR for spike (x-axis) and nonspike (y-axis) for a) FET-based scores (p values), b) observational ATEs, c) AIRIVA-based ATEs via conditional generation, d) AIRIVA-based ATEs via counterfactuals.

% \subsubsection{Treatment effect estimation with AIRIVA can disentangle label-specific TCRs}

% In this Section, we demonstrate how AIRIVA can identify label specific TCRs, even when these are highly correlated in the observed repertoires. We could consider AIRIVA as an improved FET that accounts for potential confounding, e.g., HLA and depth.


% \paragraph{Fig} effect size per TCR for spike (x-axis) and nonspike (y-axis) for a) FET-selection, b) ATE-selection, c) Input-gradients for feedforward NN.

% Take-aways:
% \begin{enumerate}
% 	\item axis alignment of ATE along spike/nonspike latents
% 	\item greater match with MIRA hits in top K from ATE vs baselines?
% \end{enumerate}

% The oracles illustrates what is possible to achieve when we have perfect knowledge of underlying confounders/causal relations underneath.
% %  when we have perfect controls and do not have confounders that bias the ATE (differences in expectations) or FET (assignments to case/controls).  If we have perfect assignments, to cases and controls, we do not need a model and the FET/empATE is sufficient.

% % TED: What's interesting is that to do the FETs above we needed to drop the healthy controls from the NS estimates and drop the covid+ from the S estimates.  Both contaminate the effect estimations in undesirable ways.  For NS estimation, the healthy controls overestimate Spike signal and for S estimation the Covid samples add NS noise.  Both of these effects are seen in the correlation plots we originally showed between the spike / nonspike neg-logp plots.

% % TED: we can compare the perfect FET/empATE results with our model based ATEs that use more data and importantly, contaminated labels.  We should show easily the robustness to having a model such as AIRIVA "clean" up the contamination by learning to disentangle the signal.


% % TED: First, we explain this with diagrams indicating sets of TCRs for spike/ nonspike and how not having perfect controls is an issue when we do not have a model.  Second, there are a few arguments for why what we are doing makes sense.  The easiest is a sample size argument.  Even with perfect knowledge regarding case controls we create smaller and smaller populations for FET / empATE when the number of factors goes up.  The other main argument is debiasing.  By adding factors, such as depth and HLAs that introduce bias into FET/empATE into AIRIVA we can debias.  And another which is related to both is the componential idea of our factorization.  As we add more targets (especially, say, all HLAs) we get fewer and fewer perfectly matched cases and controls, ie we do get each HLA in many samples but not each combination.  AIRIVA seems to be, hopefully, robust to this.



% \begin{figure*}[h!]
% 	\centering
% 	%\includegraphics[width=\linewidth]{figures/ATEs_placeholder.png}
% 	\caption{Disentanglement of Latent Factors for Disease and Risk:  (A) training and (B) holdout datasets. In both cases, a clear separation in the disease and risk dimensions are observed in the latent space. }
% 	\label{fig:counterfactuals_model}
% \end{figure*}
% \begin{figure}[h!]
% 	\centering
% 	\begin{subfigure}{0.3\textwidth}
% 		%\includegraphics[width=\textwidth]{figures/fet_naive}
% 		\caption{FET-based scores.}
% 		\label{fig:first}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{0.3\textwidth}
% 		%\includegraphics[width=\textwidth]{figures/mean_diff_naive}
% 		\caption{Group mean differences.}
% 		\label{fig:second}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{0.3\textwidth}
% 		%\includegraphics[width=\textwidth]{figures/ATE_cond_generation}
% 		\caption{AIRIVA-based ATEs via conditional generation.}
% 		\label{fig:third}
% 	\end{subfigure}

% 	\vspace{0.1cm}

% 	\begin{subfigure}{0.3\textwidth}
% 		%\includegraphics[width=\textwidth]{figures/fet_oracle}
% 		\caption{Biologically informed FET-based scores.}
% 		\label{fig:first}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{0.3\textwidth}
% 		%\includegraphics[width=\textwidth]{figures/mean_diff_oracle}
% 		\caption{Biologically informed group mean differences.}
% 		\label{fig:second}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{0.3\textwidth}
% 		%\includegraphics[width=\textwidth]{figures/ATE_counterfactuals}
% 		\caption{AIRIVA-based ATEs via counterfactuals.}
% 		\label{fig:third}
% 	\end{subfigure}

% 	\caption{Comparing TCR selection/ATE approaches}
% 	\label{fig:figures}
% \end{figure}


% \subsubsection{Treatment effect estimation with AIRIVA can identify HLA context-specific TCRs for a given antigen}\label{sec:result_hla}
% % describe cluster assignments, experimental setup, etc @Niranjani

% \paragraph{Fig} per-HLA conditional effect size per TCR for (a) spike (x-axis) and nonspike (y-axis) in A*(02/01):01 HLA  cluster, (b) not in this cluster, (c) Non spike ATEs in (y-axis) and out (x-axis) of cluster, (d) spike ATEs for the same. Ideally, what we want to see here is nonspike/spike MIRA hits respectively along each axis.

% \subsection{(AIRIVA in-silico repertoires retain label information)}
% % in-silico generation of repertoires with downstream applications such as data augmentation, ATE/CATE estimation.

% Using in-silico AIRIVA-generated repertoires yield high predictive performance, comparable to real repertoires. Below some experiment ideas we could conduct to argue this point:

% Option 1. train an ESLG/EMLG model with only in-silico AIRIVA-generated repertoires. Do we obtain similar predictive performance as a model trained on observed repertoires?

% Option 2: suppose we have limited number of observed repertoires. We train an AIRIVA model with such reduced dataset, and then train an ESLG model with (observed + in-silico) repertoires. Can we improve predictive performance of ESLG? [Skeptical, because if we have reduced number of repertoires, that will impact the quality of the learned AIRIVA model].

% Option 3: train an AIRIVA model, and then generate a much smaller set of in-silico repertoires. The hope is that AIRIVA can learn to generate "unbiased" datasets, such that with same amount of data, in-silico repertoires exhibit a cleaner signal.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TRASH %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % We train the AIRIVA model with a data set of 972 individuals with MS and 2789 individuals in the control group for the training set. The test set has a total of 3364 individuals (374 cases and 2990 controls). We use disease, risk alleles and depth as factors of interest. In addition we are choosing the top 20 HLAs that maximize the difference in frequency of occurrence between controls and cases. The original size of the TCR repertoires is in the order of millions. Following \cite{emerson2017immunosequencing} we select the top most significant TCR using Fisher's exact test (FET). In particular, we choose the top most significant 5000 TCRs with respect to the disease.

% %We train the AIRIVA model by maximizing the ELBO in \eqref{eq:elbo}. We use 700 minimum epochs, the Adam optimizer with a learning rate of $e^{-4}$, 3 encoder layers, 2 decoder layers, 256 hidden dimensions and 10 residual latents. We implemented and trained the model using PyTorch Lightning.



% %\subsection{Disentangling disease and risk with the AIRIVA model}

% % To validate the disentanglement achieved by the model, we visualize the latent factors learned for disease and risk. Figure \ref{fig:countefactuals_model} shows samples from the posterior distribution over the disease and risk latent factors (risk HLAs in this case) i.e., $q(z_{disease} | \textbf{x})$ and $q(z_{HLA} | \textbf{x})$ are plotted against each other. Figure \ref{fig:countefactuals_model} (A) shows the results for the training samples and Figure \ref{fig:countefactuals_model} (B) shows the results for the test. As it is evident, the latent space of the model is able to recover and disentangle the four expected subpopulations that result of the combinations of disease and risk. It is precisely this disentanglement which allows to generate counterfactuals in which the generative direction of the model is use sample synthetic repertoires by changing one factor at a time.

% %Once we have demonstrated that risk are disease are properly disentangled by the model, we analyze the effect of this property in the generation of counterfactuals for both factors. We fist train two separates logistic regression classification models on the observed TCR data to infer the disease (MS) and the presence of risk HLAs. For each TCR repertoire, two counterfactuals are generated one for disease an other for HLA and the logits are computed for both the original data and the counterfactuals. Figure \ref{fig:countefactuals_model} (A) illustrated the values of logits in for the disease classification model. Figure \ref{fig:countefactuals_model} (B) shows the same for the HLA model. In both figures we highlight and example of the effect of swapping the disease (blue points) or the HLA labels (orange points), and the corresponding logits from the classifiers are plotted against that of the original factual input. Deviation from the diagonal line indicates a change in classification outputs on the counterfactuals: Figure~\ref{fig:countefactuals_model} (A) shows that the disease-counterfactuals cause a strong switching of disease predictions (e.g., case to control and control to case as indicated by arrows); Figure \ref{fig:countefactuals_model} (B) shows a similar but pronounced trend for HLA counterfactuals while disease counterfactuals do not influence the HLA predictions much (note the proximity to the diagonal), implying that the HLA counterfactuals do not considerably interfere the disease signals in the inputs. %Figure \ref{fig:countefactuals_model} (C) and Figure \ref{fig:countefactuals_model} (D) same figures for depth.



% %\subsection{Robust prediction of disease label with counterfactual augmentation}

% %This experiment illustrates the utility of generating counterfactuals when the goal is to predict disease. Following XXX, we use an Exact Match logistic regression as baseline model. This is a special type of logistic regression trained with the Adam optimizer where the model weights are clipped to be positive after each iteration. We train it on the original dataset and augmented versions of the training data where different types of counterfactuals generated with AIRIVA are added. The goal is to analyze the impact of the counterfactual data augmentation on the final classification results.

% %Because the addition of counterfactuals has a balancing effect, we analyze the resutls from a robustness point of view by leveraging average test performance and behviour on subpopulation level.

% %All the logistic regression models in this section are tuned using 50 Bayesian optimization trials. We optimze the batch size $(1, 3761)$, the learning rate ($e^{-4}$, $e^{-3}$) and weight decay ($e^{-5}$, $e^{-2}$). We also clamped weights of the logistic model since we assume that TCRs can only have a positive effect in the probability of disease.

% %%%%%% METRICS %%%%%%%%

% %%%%%%%%%%%%%%%%%%%%%%%%%%%% TRASH %%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %\begin{enumerate}
% %\item Two-step Fisher Exact Test as feature selection + train separate logistic regression (LR) classifiers for each task (2 baselines actually) ESLG (published by Adaptive) / EMLG
% %\item Two-step Fisher Exact Test as feature selection + Multi-task Feedforward neural network (same architecture as AIRIVA, but without reconstruction loss nor KL regularization, just predictive loss term) - multi-task EMLG
% %\item "Oracle" model: this model is using MIRA data, whereas any other baseline only assumes repertoire count data (since this uses additional wet lab data, not a true baseline, but rather an upper bound of the best performance we can achieve)
% %\end{enumerate}



==> sections/tikz_counterfactual_graph.tex <==

\begin{tikzpicture}
    \node [nodeobserved] (x) {$\xv$};
    \node [nodeobserved, below = of x] (y1) {$\Y^\l_1$};
    \node [nodeobserved, below = of y1] (y2) {$\Y^\l_2$};
    \node [node, right = of x] (zres) {$\zv_{\epsilonv}$};
    \node [node, right = of x] (z2) {$\zv^2_y$};
    \node [node, right = of y1] (z1) {$\zv^1_y$};
    % \node [node, above = of x](zx) {$\mathbf{z}_x$};
    % \node [node, left = of zx](zd) {$\rvz_d$};
    % \node [node, right = of zx] (zy) {$\rvz_y$};
    % \node[semifill={gray!50,ang=45}] (y) {$\Y^\l$};
    % \node [nodeobserved,left color=white,right color=gray!50] (y) {$\Y^\l$};
% \node[yshift=-1.5cm, draw, circle, fill=gray!40, shading=axis, shading angle=90, minimum size=3em] (y) {$\Y^\l$};

    % \node [node, below = of y] (z) {$\zv^\l_y$};
    % \node [nodeobserved, left = of z] (x) {$\xv_j$};
    % \node [node, left = of y] (zres) {$\zv_{\epsilonv}$};
    % \plate [] {plate1} {(y)(z)} {$\d$};
    % \plate [] {plate1} {(x)} {$J$};

    % \draw [arrow] (y) -- (z);
    % \draw [arrow] (z) -- (x);
    % \draw [arrow] (zres) -- (x);
    % \draw[->, dashed, bend right] (x) to (z);
    % \draw[->, dashed, bend right] (x) to (zres);
    % \draw[->, dashed, bend right] (z) to (y);
\end{tikzpicture}

==> sections/tikz_covid_graphical_model.tex <==
		\begin{tikzpicture}
			% \node [nodeobserved] (x) {$\mathbf{x}$};
			% \node [node, above = of x](zx) {$\mathbf{z}_x$};
			% \node [node, left = of zx](zd) {$\rvz_d$};
			% \node [node, right = of zx] (zy) {$\rvz_y$};
			\node [nodeobserved,left color=white,right color=gray!50] (y1) {$\Y^{\text{s}}$};
			\node [nodeobserved,right = of y1, left color=white,right color=gray!50] (y2) {$\Y^{\text{ns}}$};
			\node [nodeobserved,right = of y2] (d) {$\Y^{\text{d}}$};
   % \node[yshift=-1.5cm, draw, circle, fill=gray!40, shading=axis, shading angle=90, minimum size=3em] (y) {$\Y^\l$};
   
			\node [node, below = of y1] (z1) {$\zv^{\text{s}}$};
			\node [node, below = of y2] (z2) {$\zv^{\text{ns}}$};
			\node [node, below = of d] (z3) {$\zv^{\text{d}}$};
			\node [nodeobserved, below = of z1] (x) {$\xv$};
			\node [node, left = of z1] (zres) {$\zv_{\epsilonv}$};
			% \plate [] {plate1} {(y)(z)} {$\d$};

			\draw [arrow] (y1) -- (z1);
			\draw [arrow] (y2) -- (z2);
			\draw [arrow] (d) -- (z3);
			\draw [arrow] (z1) -- (x);
			\draw [arrow] (z2) -- (x);
			\draw [arrow] (z3) -- (x);
			\draw [arrow] (zres) -- (x);
            \draw[->, dashed, bend right] (x) to (z1);
            \draw[->, dashed, bend right] (x) to (z2);
            \draw[->, dashed, bend right] (x) to (z3);
            \draw[->, dashed, bend right] (x) to (zres);
            \draw[->, dashed, bend right] (z1) to (y1);
            \draw[->, dashed, bend right] (z2) to (y2);
            \draw[->, dashed, bend right] (z3) to (d);
	   \end{tikzpicture}

==> sections/tikz_hsv_graphical_model.tex <==
		\begin{tikzpicture}
			% \node [nodeobserved] (x) {$\mathbf{x}$};
			% \node [node, above = of x](zx) {$\mathbf{z}_x$};
			% \node [node, left = of zx](zd) {$\rvz_d$};
			% \node [node, right = of zx] (zy) {$\rvz_y$};
			\node [nodeobserved,left color=white,right color=gray!50] (y) {$\Y^\l$};
   % \node[yshift=-1.5cm, draw, circle, fill=gray!40, shading=axis, shading angle=90, minimum size=3em] (y) {$\Y^\l$};
   
			\node [node, below = of y] (z) {$\zv^\l_y$};
			\node [nodeobserved, left = of z] (x) {$\xv$};
			\node [node, left = of y] (zres) {$\zv_{\epsilonv}$};
			\plate [] {plate1} {(y)(z)} {$\d$};

			\draw [arrow] (y) -- (z);
			\draw [arrow] (z) -- (x);
			\draw [arrow] (zres) -- (x);
            \draw[->, dashed, bend right] (x) to (z);
            \draw[->, dashed, bend right] (x) to (zres);
            \draw[->, dashed, bend right] (z) to (y);
	   \end{tikzpicture}

==> sections/trash.tex <==
% % AIRIVA can generate realistic in-silico repertoires. The characteristics of AIRIVA-generated TCR count repertoires are similar to the real repertoires when we intervened on labels.
% % \begin{enumerate}
% %     \item Effect of intervening on binary labels: Poisson rate in latent space. In Appendix, MIRA hits for the corresponding label are activated.
% %     \item Effect of intervening on depth: augment total sum of TCR counts in repertoire.
% %     \item Effect of intervening on age: proportion of CD4/CD8 consistent with reality.
% % \end{itemize}


%  %  \begin{table}[h!]
% 	%  \footnotesize
% 	%  \begin{center}
% 	% 	 \begin{tabular}{c||c|c}
% 	% 		 \toprule
% 	% 		 %& \multicolumn{2}{c|}{LG-based models} & \multicolumn{2}{c}{AIRIVA} \\
% 	% 		 %\midrule %\cmidrule{1-2} \\
% 	% 		  & AUC Spike & AUC Nonspike \\
% 	% 		 \midrule
% 	% 		 Factuals  & $ 0.00 \pm 0.0$ &  $ 0.00 \pm 0.0$ \\
%  %              Ctf (all)  & $ 0.00 \pm 0.0$ &  $ 0.00 \pm 0.0$ \\
%  %              Ctf (controls)  & $ 0.00 \pm 0.0$ &  $ 0.00 \pm 0.0$ \\
%  %              Ctf (vaccinated)  & $ 0.00 \pm 0.0$ &  $ 0.00 \pm 0.0$ \\
%  %              Ctf (sick)  & $ 0.00 \pm 0.0$ &  $ 0.00 \pm 0.0$ \\
% 	% 		 %\midrule
% 	% 		 \bottomrule
% 	% 	 \end{tabular}
% 	% 	 \caption{Quantitative evaluation of counterfactuals.}\label{tab:per-group}
% 	%  \end{center}
%  % \end{table}

% % \begin{figure}[h!]
% % 	\centering
% % 	\begin{subfigure}{0.45\textwidth}
% % 		\includegraphics[width=\textwidth]{figures/latent_space/fig1a_annotated}
% % 		\caption{Stratified by subgroups.}
% % 		\label{fig:latent1}
% % 	\end{subfigure}
% % 	\begin{subfigure}{0.45\textwidth}
% % 		\includegraphics[width=\textwidth]{figures/latent_space/fig1b_annotated}
% % 		%\includegraphics[width=\textwidth]{figures/latent_space_vaccines2.png}
% % 		\caption{Stratified by vaccine type.}
% % 		\label{fig:latent2}
% % 	\end{subfigure}
% % 	\caption{\textbf{Latent space representation}. Each point corresponds to one sample $z$ from the posterior $q(z|x)$. On the sides, we show marginal posterior distributions as continuous lines, and predictive priors as dashed lines. (a) Predictive priors $p(z_y|y)$ for each combination of labels $y$ are represented as one ellipse corresponding to 1 standard deviation. (b) Latent space for the vaccinated subgroup (coloured) stratified by different vaccine types; samples for other subgroups are shown in grey.}
% % 	\label{fig:latent_space}
% % \end{figure}

% PEARSON CORRELATION

% Figure~\ref{fig:pearsoncorrelation} shows the Pearson correlation between the estimated spike and nonspike treatment effect for the different baselines. Based on domain expertise, we know that exposure to the spike and nonspike proteins engage completely different sets of TCRs. A good approach for classification of antigen-specific TCRs should thus exhibit zero correlation between both quantities. Interestingly, both naive and matched baselines exhibit non-zero correlation, whereas AIRIVA-based ATEs exhibit correlation values closer to zero for both conditional generation and counterfactual generation.

% \begin{figure}
% 	\centering
% 	\includegraphics[width=1.0\linewidth]{figures/mira_classification/pearson_correlation}
% 	\caption{Person correlation between group mean differences for spike and nonspike labels averaged across multiple AIRIVA runs (5 random seeds and 5 different subsampling fractions for the positive-labels). We want these two score to be uncorrelated (best value is zero). }
% 	\label{fig:pearsoncorrelation}
% \end{figure}

% ABLATION

% Figure~\ref{fig:tcr-classification} shows quantitative results comparing these 3 approaches as we increase the input-dimensionality (number of TCRs) and subsample the number of positive-labels available in the training set. In the classification task of spike-specific TCRs (first row), the matched approach is the best method, ATEs computed via counterfactuals from AIRIVA are almost as good as the matched approach, followed by ATE via conditional generation with AIRIVA and the naive baseline. Regarding the classification task of non-spike TCRs, ATEs estimated with AIRIVA are as bad as the naive approach. This is due to our incapacity to generate realistic non-spike only repertoires (the unseen class in the train set). Further inductive biases need to be included in the model in order to constraint the solution space such as the decoder is able to generate repertoires never observed in train.


% \begin{figure*}[]
% 	\centering
% 	\includegraphics[width=\linewidth]{figures/mira_classification/fig6_ablation_MIRA_classification_performance}
% 	\caption{Antigen-specific TCR classification evaluated using wetlab data from the MIRA panel. Classification of spike-specific TCRs (first row) and nonspike-specific TCRs (second row). We compare the two baselines, naive approach (uses all data available) and matched approach uses subsets of the data to better match cases to controls, against AIRIVA average treatment effect estimation by either conditional generation or counterfactual generation. We rely on integrated precision at top-k TCRs.
% 	}
% 	\label{fig:tcr-classification}
% \end{figure*}


% ATE ESTIMATION

% \begin{figure*}[h!]
% 	\centering
% 	\begin{subfigure}{0.24\textwidth}
% 		\includegraphics[width=\textwidth]{figures/GMD_all_independent}
% 		\caption{Naive cases to controls}
% 		\label{fig:first}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{0.24\textwidth}
% 		\includegraphics[width=\textwidth]{figures/mean_diff_oracle}
% 		\caption{Matched cases to controls}
% 		\label{fig:second}
% 	\end{subfigure}
% 	\hfill
% 	\begin{subfigure}{0.24\textwidth}
% 		\includegraphics[width=\textwidth]{figures/ate_counterfactual_AIRIVA}
% 		\caption{AIRIVA Counterfactuals}
% 		\label{fig:third}
% 	\end{subfigure}
%  \begin{subfigure}{0.24\textwidth}
% 		\includegraphics[width=\textwidth]{figures/mean_diff_oracle}
% 		\caption{Intervened AIRIVA Ctfs. PLACEHOLDER.}
% 		\label{fig:third}
% 	\end{subfigure}
% 	\caption{Estimation of Treatment Effects by (a) Naive approach: splitting all available individuals into cases and controls for each positive label, regardless of any unobserved confounder, (b) selecting subsets in the dataset to better match between cases and controls (by accounting for known correlations for example), (c) using a model such as AIRIVA to impute the potential outcomes, and estimate average treatment effects via counterfactual generation. In this example, we estimate the effect of the spike antigen by taking all vaccinated individuals, and compute their corresponding counterfactual of removing the effect of vaccine.}
% 	\label{fig:figure_ATEs}
% \end{figure*}


% \begin{figure}[]
% 	\centering
% 	%\includegraphics[width=\linewidth]{diagrams/intro_airiva.png}
% 	%\includegraphics[width=3cm]{example-image-c}
	
% 	\begin{subfigure}{0.45\linewidth}
% 		\includegraphics[width=1.0\linewidth]{figures/intro/covid_virus}
% 		\caption{SARS-CoV-2 structure}
% 		\label{fig:covid_virus}
% 	\end{subfigure}
% 	\begin{subfigure}{0.45\linewidth}
% 		\includegraphics[width=\textwidth]{figures/intro/covid_virus_labels}
% 		\caption{AIRIVA label definition}
% 		\label{fig:labels_def}
% 	\end{subfigure}
% 	\caption{Domain knowledge for SARS-CoV-2
% 	}
% 	\label{fig:virus_labels}
% \end{figure}

 % Describe pipeline and training strategy.
% 1. Run FET-preprocessing step to reduce input dimensionality
% 2. Train an AIRIVA model with Spike+Non-spike+Age+Depth labels
% Describe hyperparameter optimization and model selection strategies 



% \begin{figure}[h!]
% 	\centering
% 	\includegraphics[width=\linewidth]{figures/condgen/effect_age.png}
% 	\caption{Proportion of CD4/CD8 of in-silico repertoires when intervening on age.}
% 	\label{fig:effect_age}
% \end{figure}


% \begin{figure}[hb!]
% \centering
%     %\begin{tikzpicture}
%     %\node [node_no_draw] (y1) {$y_1$};
%     %\node [node_no_draw, below right = of y1] (y2) {$y_2$};
%     %\node [node_no_draw, below = of y1, yshift=0.3cm] (x) {$\mathbf{x}$};

%     %\draw [arrow] (y1) -- (x);
%     %\draw [arrow] (y2) -- (x);
%     %\draw [arrow] (y1) -- (y2);
%     %\end{tikzpicture}\\
%     \begin{tikzpicture}
%         \node [node_no_draw] (c) {$\mathbf{c}$};
%         \node [node_no_draw, below left = of c] (y1) {$y_1$};
%         \node [node_no_draw, below right = of c] (y2) {$y_2$};
%         \node [node_no_draw, below = of c, yshift=0.3cm] (x) {$\xv$};
%         \draw [arrow] (y1) -- (x);
%         \draw [arrow] (y2) -- (x);
%         \draw [arrow] (c) -- (y1);
%         \draw [arrow] (c) -- (y2);
%     \end{tikzpicture}
%     \caption{\textbf{Disentangled causal process with confounding}. Example causal graph in which $c$ is a confounder between labels $y_1$ and $y_2$. }
% \label{fig:causal_models}
% \end{figure}

\subsection{Synthetic Experiments}

In order to establish a proof of concept for the use of AIRIVA to learn factors of variation and estimate treatment effects in TCR repertoire data, we first consider a fully synthetic dataset in which the underlying data generating process is perfectly known. We simulate such a dataset as follows...
%We generate data according to two different causal graphs, to evaluate the ability of AIRIVA to identify and correct for mediation bias, confounders...

Comparision of true ATE versus estimated ATE between AIRIVA and GMD. Other ways to rank TCRs such as pvalue or EMLG weights in Appendix. Highlight that we are the only method that enables estimation of counterfactuals and ITEs on top of ATEs.

\begin{figure}[t]
	\centering
	% \begin{subfigure}{0.23\textwidth}
	% 	\includegraphics[width=\textwidth]{figures/synthetic_data/synth_GMD.png}
	% 	\caption{Group Mean Differences}
	% 	\label{fig:synth_GMD}
	% \end{subfigure}
	% \hfill
	% \begin{subfigure}{0.23\textwidth}
	% 	\includegraphics[width=\textwidth]{figures/synthetic_data/synth_AIRIVA.png}
	% 	\caption{AIRIVA}
	% 	\label{fig:synth_AIRIVA}
	% \end{subfigure}
        \begin{subfigure}{0.23\textwidth}
		%\includegraphics[width=\textwidth]{figures/synthetic_data/synth_GMD.png}
		\caption{Generative Process}
		\label{fig:synth_GMD}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.23\textwidth}
		\includegraphics[width=\linewidth]{figures/final/airiva_toy.png}
		\caption{ATE estimation}
		\label{fig:synth_AIRIVA}
	\end{subfigure}
	\caption{{Estimation of ATE with AIRIVA in a controlled scenario. (PLACEHOLDER)}}
	\label{fig:synthetic_ATEs}
\end{figure}

\subsection{Notes for Related Work}

\cite{scholkopf2012causal} introduces the independent mechanism assumption, the notion  that each elementary element can be changed without affecting others.


\subsection{Further Related Work}

\paragraph{Feature selection for TCR-based diagnostics} The large space of potentially relevant TCRs from a set of case and control repertoires (O(100M)) compared to the small number of disease-associated TCRs ($\leq 1\%$ of each repertoire) necessitates filtering to a smaller set of relevant TCRs to facilitate downstream classification. For example, a one-tailed Fisher's Exact Test (FET) with a p-value threshold can be employed to reduce the relevant TCRs to a set of these \textit{enhanced sequences} which are over-represented in cases vs. controls. These sequences can be input to downstream classification methods, for example, training generative binary classification models~\citep{emerson2017immunosequencing}, logistic regression models~\citep{snyder2020magnitude, gittelman2021diagnosis,elyanow2022t}, logistic growth models \citep{greissl2021immunosequencing}, or random forest models \citep{DeNeuter2018, Liu2019}---to produce a disease diagnostic.

However, TCR selection using a statistical test doesn't capture differences between case and control populations caused by factors other than the disease label. These can include imbalances in HLA frequency, age, or sequencing depth between cases and controls. It is therefore desirable to cast a wide-enough net during the TCR pre-selection process and allow downstream models to not only correct for confounding effects due to pre-selection, but also to disentangle other factors of variation.
% JG: TCR selection by any statistical test ignores potential differences between the groups that are caused by external factors different to the disease label. For instance, if all controls are young patients and all cases are old patients, the test may produce false positives, which will result in a poor biomarker identification strategy.

\textbf{Deep Learning for Immunomics}. Modern applications of deep learning to immunomics can be generally split into three categories: predicting TCR-pMHC binding and generating pMHC-specific TCRs, predicting TCR generation probability, and predicting TCR repertoire-level labels---see \cite{annurev-chembioeng} for an overview. The prediction of TCR-pMHC binding and TCR generation probabilities have been extensively explored using several deep learning approaches, including: FNNs \citep{Springer2020, Fischer2020, Montemurro2021}, CNNs \citep{Moris2020, Jokinen2022}, and VAEs \citep{Sidhom2021, Davidsen2019, Isacchini2020}.
%AE~\citep{min2022learning},
%, and transfer learning \citep{Lu2021}.

 %  \begin{table}[h!]
	%  \footnotesize
	%  \begin{center}
	% 	 \begin{tabular}{c||c|c|c}
	% 		 \toprule
	% 		 %& \multicolumn{2}{c|}{LG-based models} & \multicolumn{2}{c}{AIRIVA} \\
	% 		 %\midrule %\cmidrule{1-2} \\
	% 		 Model & Sensitivity & AUCROC & Stability \\
	% 		 \midrule
	% 		 AIRIVA   & $ 0.63 \pm 0.05$ &  $0.80 \pm 0.02$ & $0.02 \pm 0.01$ \\
	% 		 AIRIVA+d & $ 0.69 \pm 0.06$  & $0.81 \pm 0.04$ & $0.12 \pm 0.07$ \\
 %        %AIRIVA+d+a & $ 0.0 \pm 0.0$  & $0.0 \pm 0.0$ & $0.0 \pm 0.0$ \\
	% 		 %\midrule
	% 		 %Predictive AIRIVA & $0.6 \pm 0.01$ & $0.6 \pm 0.01$ & $0.6 \pm 0.01$ \\
	% 		 \bottomrule
	% 	 \end{tabular}
	% 	 \caption{Predictive performance and instability averaged across top-5 best AIRIVA models. We report sensitivity group average at 99\% specificity, Area Under Concentrated Operating Curve (AUCROC) group average~\cite{swamidass_croc_2010}, and instability range when stratifying the holdout set by different depth bins.}\label{tab:per-group}
	%  \end{center}
 % \end{table}


 % \begin{figure}[]
% 	\centering
% 	\begin{subfigure}{0.45\textwidth}
% 		%\includegraphics[width=\textwidth]{figures/latent_space/fig1a_annotated}
%         %\includegraphics[width=\textwidth]{figures/covid/latent_covid_best.png}
%         \includegraphics[width=\textwidth]{figures/final/best_run/latent_holdout.png}
% 	\end{subfigure}
% 	\caption{\textbf{Latent space for SARS-CoV-2}. Each point corresponds to one sample $\sz$ from the posterior $q(\zv|\xv)$ in holdout. On the sides, we show the marginal posteriors as continuous lines, and predictive priors as dashed lines. Predictive priors $p(\zv_y|\yv)$ for each combination of labels are represented as ellipses, each circle denoting one standard deviation.}
% 	\label{fig:latent_space_COVID}
% \end{figure}

% \begin{figure}[h!]
% 	\centering
% 	\begin{subfigure}{0.43\textwidth}
%       \includegraphics[width=\textwidth]{figures/final/best_run/latent_space_vaccine3}
% 	\end{subfigure}
%         \begin{subfigure}{0.43\textwidth}
%         \includegraphics[width=\textwidth]{figures/final/best_run/vaccine1.png}
%         \end{subfigure}
% 	\caption{\textbf{Latent space stratified by vaccine type}. Each point corresponds to one sample $\sz$ from the posterior $q(\zv|\xv)$. On the sides, we show marginal posterior distributions as continuous lines, and predictive priors as dashed lines. Latent space for the vaccinated subgroup (coloured) stratified by different vaccine types; samples for other subgroups are shown in grey.}
% 	\label{fig:vaccine_latent_space}
% \end{figure}

% \begin{figure}[th]
%     \centering
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{figures/ML4HC/HSV/roc_curves/roc_hsv1_all.png}
%         \subcaption{(a) HSV-1 for All}\label{fig:hsv1}
%     \end{minipage}
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{figures/ML4HC/HSV/roc_curves/roc_hsv1_conditioned_hsv2_negative.png}
%         \subcaption{(b) HSV1 for HSV2-negative}\label{fig:hsv1_cond_hsv2_neg}
%     \end{minipage}
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{figures/ML4HC/HSV/roc_curves/roc_hsv1_conditioned_hsv2_positive.png}
%         \subcaption{(c) HSV1 for HSV2-positive}\label{fig:hsv1_cond_hsv2_pos}
%     \end{minipage}

%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{figures/ML4HC/HSV/roc_curves/roc_hsv2_all.png}
%         \subcaption{(d) HSV2 for All}\label{fig:hsv2}
%     \end{minipage}
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{figures/ML4HC/HSV/roc_curves/roc_hsv2_conditioned_hsv1_negative.png}
%         \subcaption{(e) HSV2 for HSV1-negative}\label{fig:hsv2_cond_hsv1_neg}
%     \end{minipage}
%     \begin{minipage}{0.32\textwidth}
%         \centering
%         \includegraphics[width=1\textwidth]{figures/ML4HC/HSV/roc_curves/roc_hsv2_conditioned_hsv1_positive.png}
%         \subcaption{(f) HSV2 for HSV1-positive}\label{fig:hsv2_cond_hsv1_pos}
%     \end{minipage}
    
%     % \begin{minipage}{0.48\textwidth}
%     %     \centering
%     %     \includegraphics[width=1\textwidth]{figures/ML4HC/HSV/roc_hsv1.png}
%     %     \subcaption{(a) HSV1 Prediction Task}\label{fig:hsv1}
%     % \end{minipage}
%     % \begin{minipage}{0.48\textwidth}
%     %     \centering
%     %     \includegraphics[width=1\textwidth]{figures/ML4HC/HSV/roc_hsv2.png}
%     %     \subcaption{(b) HSV2 Prediction Task}\label{fig:hsv2}
%     % \end{minipage}
%     \caption{ROC Curves for HSV disease prediction models. First row: HSV1 Prediction Task; Second row: HSV2 Prediction Task}
% \end{figure}
